Data Privacy in Trigger-Action Systems

Trigger-action platforms (TAPs) allow users to connect independent web-based or IoT services to achieve useful automation. They provide a simple interface that helps end-users create trigger-compute-action rules that pass data between disparate Internet services. Unfortunately, TAPs introduce a large-scale security risk: if they are compromised, attackers will gain access to sensitive data for millions of users. To avoid this risk, we propose eTAP, a privacy-enhancing trigger-action platform that executes trigger-compute-action rules without accessing users' private data in plaintext or learning anything about the results of the computation. We use garbled circuits as a primitive, and leverage the unique structure of trigger-compute-action rules to make them practical. We formally state and prove the security guarantees of our protocols. We prototyped eTAP, which supports the most commonly used operations on popular commercial TAPs like IFTTT and Zapier. Specifically, it supports Boolean, arithmetic, and string operations on private trigger data and can run 100% of the top-500 rules of IFTTT users and 93.4% of all publicly-available rules on Zapier. Based on ten existing rules that exercise a wide variety of operations, we show that eTAP has a modest performance impact: on average rule execution latency increases by 70 ms (55%) and throughput reduces by 59%.

==> background.tex <==
\section{Background}\label{sec:background}
% brief overview of trigger-compute-action: say something that new version supports computation, whiel Zapier always supported
% motivation of security/privacy issues for data

% \begin{figure*}[t!]
%   \centering
%   \hpagess{0.5}{0.5}{
%     \centering\includegraphics[width=\textwidth]{images/tas.png}
%     \textbf{(a)}
%   }{
%     \centering\vspace{-2.75cm}
%     \includegraphics[width=\textwidth]{images/otap.png}
%     \textbf{(b)}
%   }
%   \caption{Architecture overview of current trigger-action system
%     (\textbf{a}) and $\stap$ (\textbf{b}). }
% \label{fig:tas}
% \end{figure*}

\begin{figure}[t!]
  \centering \includegraphics[width=0.46\textwidth]{images/tas_2.png}
    \caption{Overview of current trigger-action systems.}
      %(\textbf{a}) and $\stap$ (\textbf{b}). }
\label{fig:tas}
\end{figure}

% We discuss background information on trigger-action systems, introduce our
% abstract computational model of trigger-compute-action programs, and finally
% discuss the privacy risks of TAPs.

% \subsection{Trigger-action systems}
Trigger-action systems allow stitching together disparate online services using
a trigger-compute-action paradigm to automate different tasks. There are three
main components of the system: trigger services (TSs), action services (ASs),
and a trigger-action platform (TAP). We also explicitly mention another
computing component: the client's device used to interface with the trigger-action system. \figref{fig:tas} shows the interactions between different components.


%The diagram showing the interactions between different components are given in the\fixme{left and right?} top figure of~\figref{fig:tas}.


% Figure~\ref{fig:tas} shows an architectural overview of trigger-action systems. At a high level, they stitch together disparate online services of a user and provide them the ability to create and run trigger-compute-action rules of the form: ``IF my location is within 50 meters of my home, THEN open the door.''  These systems are useful in automating various tasks, and have been especially well-suited to programming smart homes~\cite{ur2014practical}. Trigger-action systems currently have millions of users and user-created rules.


%Trigger-compute-action programming is new paradigm of programming where an end user can
%programmatically connect a trigger service (TS) with an action service (AS),
%such that when an event occurs at the trigger service, the action service is
%notified with a specific command to execute. Typically such rules look like ``If
%(trigger) then (action)'' format, for example, ``IF the thermostat's temperature
%raises above 80$^{\circ}$F THEN turn off the heater''. Given a plethora of trigger
%and action services available nowadays, it is very hard for every trigger
%service to be compatible with every other action services. Therefore,
%trigger-action platforms (TAPs) are launched that help connect such independent
%trigger and action services by sitting in the middle and providing a layer of
%abstraction to trigger and action services. There are many commercial TAPs
%available now with millions of users, such as IFTTT, Zapier, and Microsoft Flow,
%to name a few. For this paper we will focus on two most popular TAPs: IFTTT and
%Zapier.  Modern TAPs allow users to program even complex automation rules that
%modify the trigger event and then connect it to one (or multiple) action
%event(s)\footnote{None of the commercial TAPs supports multiple triggers,
%  possibly to avoid trigger synchronization overheads.}.


% \rcnote{Zapier allows paths where the TAP will send the action to specific AS
%   given the condition. We can in theory support that as well, but require some
%   overhead: send the message to every AS. We should add that to discussions.}


% \begin{algorithm}
% \caption{Trigger-Action platform's Automation Rule Model}\label{alg1}
% \begin{algorithmic}
% \Function{Rule}{Trigger.data} 

%     \STATE $time \gets \text{current time}$
    
%     \IF {$f_1(\text{Trigger.data}, time)$} 
            
%         \STATE $\text{Action.data} \gets f_2(\text{Trigger.data}, time)$
        
%         \STATE Action.perform()
        
%     \ENDIF 

% \EndFunction
% \end{algorithmic}

% \end{algorithm}

%\rcnote{Add some description to outline the differences of IFTTT and Zapier and show that our model still fits it.}

\paragraph{Trigger and action services.} These are online services for IoT or
web applications.  There is a plethora of such services available nowadays.
Examples include Instagram, Slack, GMail, Amazon Alexa, Samsung SmartThings,
GE's
Geneva,\footnote{https://www.geappliances.com/ge/connected-appliances/ranges-ovens-cooking.htm}
and many others. Most of these services provide REST APIs to send and receive
data.  The services typically support OAuth protocol~\cite{oauth}, which is used
by the client to delegate authorization to a third party, such as a TAP, to
communicate with these services.

% They are
% REST-based services and are secured using the OAuth protocol --- any entity
% wishing to access the data and actions of these services must be authorized by
% the user via OAuth.
% generates or posses sensitive user data.  The examples include 
% Instagram, Slack, GMail, Amazon Alexa, Samsung SmartThings, or GE's
% Geneva\footnote{https://www.geappliances.com/ge/connected-appliances/ranges-ovens-cooking.htm}.
% refer to of a user, and they represent sensitive data and devices. Examples
% include Instagram, Slack, GMail, Samsung SmartThings, etc. They are REST-based
% services and are secured using the OAuth protocol --- any entity wishing to
% access the data and actions of these services must be authorized by the user via
% OAuth.

\paragraph{Trigger-action platform.} 
Trigger-action platforms (TAPs) serve as a hub. Commercial TAPs are compatible
with hundreds of trigger and action services, allowing each trigger or action
service to focus on building their own REST APIs without worrying about
compatibility with each other. % Indeed, a hallmark of trigger-action systems is
% that they enable otherwise unconnected services to talk with each other.

In addition to connecting trigger and action services, modern TAPs also allow
performing non-trivial computation over the trigger data. The ability to modify
the trigger data provides a great flexibility for TAPs to achieve compatibility
between trigger and action services (e.g., a rule that pushes events from one
calendar app to another where both have different date formats). TAP operations
are also used to decide whether or not the TAP should send a message to the action
service (e.g., is the location within $50$ meters of another reference
value). % In~\secref{sec:abstract-model} we present results from a systematic
% survey of two systems: IFTTT and Zapier, and show that they support a variety of
% computations on trigger data. 
While systems like Zapier have explicitly supported computation on trigger
data~\cite{zapier:filter, zapier:formatter}, systems like IFTTT have recently
started to expose their computing interface to
end-users~\cite{IFTTT:applet}. Thus, trigger-action systems are actually
\emph{trigger-compute-action} systems. We use these two terms interchangeably
throughout the paper.


\paragraph{Client device.} This is a user's interface to a
trigger-action system. The user programs rules by selecting a trigger service
(TS), then specifies a computation on that data using a library of predefined
functions, and finally selects an action to be run on the action service
(AS). As noted before, the user also authorizes the TAP to access their online services using the client device.



% \noindent\textbf{Client:} The client is the user's interface to a trigger-action system. The user programs rules by selecting a trigger source, then specifies a computation on that data using a library of pre-defined functions, and finally selects an action to be run on the action service. The user also authorizes the trigger-action platform to their online services using the client via the OAuth protocol. 

% \noindent\textbf{Trigger-Action Platform (TAP):} The first major purpose of the TAP is to serve as an execution platform for user rules when a trigger occurs. Therefore, the computation on trigger data occurs on the TAP. These computations in general are: (1) filtering trigger data to decide whether the TAP should send a message to the action service (e.g., is my location within 50 meters of another reference value); (2) providing compatibility with action service APIs (e.g., a rule that pushes events from one calendar app to another where both have different data formats). In Section~\ref{sec:abstract-model} we present results from a systematic survey of two systems: IFTTT and Zapier, and show that they support a variety of computations on trigger data. While systems like Zapier have explicitly supported computation on trigger data \cite{zapier:filter, zapier:formatter}, systems like IFTTT have recently started to expose their computing interface to end-users \ef{put cite to JS applet}. Thus, trigger-action systems are actually \emph{trigger-compute-action} systems. We use these two terms interchangeably through the paper. 

% The second major function of the TAP is to serve as a hub. Commercial TAPs are compatible with hundreds of trigger and action services, allowing each trigger or action service to focus on building their REST APIs without worrying about compatibility with each other. Indeed, a hallmark of trigger-action systems is that they enable otherwise unconnected services to talk with each other by understanding each API.




%Before a rule can be executed in TAP, it must be set up by the user. This step
%normally involves the user selecting one trigger service and one (or multiple)
%action service(s) that need to be connected. Then the user selects a rule based
%on which the TAP will decide whether to contact the action service or not and
%what information to forward to the action service. It is to emphasize the TAP
%regularly perform non-trivial computation over the trigger data before
%forwarding it to an action service. The computation is necessary (a) to filter
%trigger to decide when to communicate to the action service, and (b) to provide
%compatibility of the APIs provided by the action service. Therefore,
%trigger-action systems are actually \emph{trigger-compute-action} system.

%Most trigger and action service require authorization from the user, and it is
%often enforced through an OAuth protocol. User authorizes TAP to communicate
%with TS and AS on behalf of the user.  Some rules might have customizable
%parameters, the user also needs to supply them during the rule-setup step.

%After the rule is set up, it will be automatically executed each time the
%trigger happens. Currently there are \fixme{two ways} to notify the TAP about
%the trigger: via pull by TAP, or via push by the trigger (when the data is
%available). Some triggers may run at period intervals, while others can be event
%driven. \todo{Given an example.}

% this is the abstract model


% \begin{enumerate}
%     \item The trigger service pushes the trigger data to the TAP when the trigger event happens.
%     \item The TAP pulls from the API of the trigger service constantly at a fixed interval (usually every 15 minutes). If the trigger happens during the interval, the trigger service responds with the trigger data; otherwise the trigger service just responds with an empty message.
% \end{enumerate}

% Once the TAP receives the trigger data, it will use it to compute predicate of the rule, $f_1$. If $f_1$ is evaluated to true, then TAP will compute $f_2$ and forward the action data to the action service though the corresponding API. If $f_1$ returns false, then no message will be sent to the action service.


\paragraph{Privacy and authenticity risks in current trigger-action systems.}
% \paragraph{Platform compromise.}
Current trigger-action platforms (TAP) receive plaintext data from a wide variety of trigger services and many of them can be sensitive.
Consider the rule: ``IF my car is near home THEN open the garage door.'' The trigger service provides updates on the car's location. The constants to the rule are the home's location and an alert radius. The trigger service periodically (e.g., every minute) sends the updated location information to the cloud-based TAP. In this simple rule, the TAP learns many types of sensitive information: the minute-wise location history of the car, and the location of the home. 

In addition to location, the sensitive information can be messages, emails, data
files, voice commands, and many more.  If the TAP is compromised, the attacker
gains access to all sensitive information that passes through the
TAP. %, making it a single point of failure.
% TAP is a cloud-service and is vulnerable to the same attacks that have plagued other cloud services, such as Target~\cite{target-breach},\rw{I just chose one report.} Equifax~\cite{equifax-breach}, US voter database~\cite{voter-breach}, and Dropbox~\cite{dropbox-breach}.
Furthermore, because commercial TAPs have millions of users with sensitive data, they are attractive targets for attackers. % Designing cloud services to be secure against breaches is a difficult problem. In this work, we show that the specific structure of current trigger-action systems allows us to split trust in a way that enables TAPs to execute rules without seeing the underlying data.


Moreover, a compromised TAP can also lie about trigger condition evaluation, and
invoke actions arbitrarily. Fernandes et al.~\cite{fernandes2018decentralized}
first noted this problem and presented DTAP, a protocol for integrity of rule
execution. However, DTAP caters to a trigger-action model where there is no
computation inside TAP. 
\as{This may sound like DTAP solves the privacy/confidentiality problem, which is the major difference with \name{}}
As discussed earlier, this is an older form of
trigger-action systems --- current systems support computation. Additionally, in
DTAP, action service checks the trigger condition, therefore the trigger data is
revealed to it. % to ensure that a malicious TAP
% is not lying about whether a trigger evaluates to true (the DTAP protocol
% requires the AS to re-check the trigger condition for rules that poll the
% trigger service). 
We observe that trigger data can be sensitive and should not be unnecessarily
revealed to the AS.

We believe such privacy and authenticity risks might be preventing
trigger-action systems from achieving their true potential. Therefore we
redesign trigger-action systems to ensure secrecy of sensitive information
without trusting the~TAP.

% its complete form to the action
% service.  % From our prior example rule above, with
% % DTAP design, a curious AS would learn the location of the child.  
% In current
% trigger-action setting, only the result of the computation is revealed, and we
% should ensure similar isolation. % Thus, providing integrity in modern TAPs
% % is still an open challenge, that we address in this work. action service




%Now the trigger service is probable a
%location provider that tracks the kid's location. The constants to the rule is
%the location of the home and some distance parameter. The trigger service
%periodically sends the location of the child every minute. The TAP from this
%rule learns a number of very sensitive information. First, TAP learns the
%location of the user's home.  Second, the TAP also learns the precise
%minute-wise location history of the child. If an attacker is able to compromise
%TAP it can learn about these sensitive information. Moreover, current TAPs does
%not provide authenticity of execution, therefore, a compromised TAP can lie to
%an action service and perform action that are not triggered by the trigger
%data. Fernandes et al.~\cite{fernandes2018decentralized} attempts to add
%integrity to trigger-action systems by ensuring TAP cannot send stale messages
%to an action service. However, in their model TAP does not apply any function on
%the trigger data, which does not fit the functionality of current commercially
%available TAPs. Moreover, the sensitive trigger data is revealed to the action
%service in to ensure integrity of the trigger, which is not safe if the action
%service is compromised. Following our example above, now a curious action
%service (which is door lock service) can observe the location history of the
%child.





% Since TAPs connect to a variety of online services and many of them are from
% private sources, some triggers will contain sensitive information that the user
% does not want to share outside of their own services. First, the \textit{trigger
%   data} (e.g. emails, personal documents) can be sensitive. In current TAP
% implementations, the data is sent to the TAP in plaintext. Therefore, if TAP is
% compromised, then the data from all triggers the user has connected to is
% inevitably leaked. Second, for some triggers, such as “door is unlocked” and
% “kid is home”, the \textit{time} when they happen is sensitive. Finally, the
% \textit{parameters} passed to the trigger can also be sensitive: consider the
% trigger “user leaves home” from a location service, it will require the user to
% pass their home address as a parameter.

%In addition to the trigger data, the trigger also learn about the action data sent to a service.
%\rcnote{working here.}
%Even if all sensitive information from the trigger is well-protected, it can still be leaked through the information sent to the action. As shown in~\figref{fig:tap}, both the predicate (whether the action is performed) and the action data are functions of the trigger data. If the attacker knows $f_1$ and $f_2$, it is possible to infer the input (trigger data) using the output (action data) and some side-channel information (such as the distribution of the input data).


% \subsection{Threat Model}

% We assume a strong attacker model: the attacker is the TAP, which means the attackers not only can monitoring the network communications between the platform and online services but also have access to the data stored inside the platform. We will adopt a semi-honest model: the platform still executes the rules correctly, but it is actively eavesdropping on the user data and might leak the user data outside of the platform. 

% Since our goal is to provide confidentiality of sensitive user data, we do not prevent the case where a compromised TAP arbitrarily changes the rule semantics or refuses to execute the rule. In addition, we assume that online services for triggers and actions are not compromised. If they are compromised, the attackers can achieve the goal without interacting with the TAP.

% Under this model, the attacker has full access to the platform, which means for each rule the following information is visible to the attacker:

% \begin{enumerate}
%     \item The messages received from the trigger service and the messages sent to the action service. Since the TAP only sends message when an action needs to be performed, it can infer the result of f1 by monitoring the network traffic. 
%     \item The time when the messages are received or sent. This should roughly equal to the time when the trigger or action happens.
%     \item The function of the rule, namely f1 and f2.
%     \item The semantics of trigger and action, which include their corresponding online services, API calls, and the parameters passed to these API calls.
% \end{enumerate}

% We also assume the attacker has some domain knowledge of the trigger and action. For example, if the trigger service is a thermostat, then the trigger data might be the user’s home temperature, which is likely to fall into a small range around 70 to 80 degrees.


% \section{Case Study}

% \subsection{IFTTT Trigger Classifications}

% To estimate the impact of the attacks, we inspected the dataset collected by Bastys et al \cite{b1}, which classified 1426 triggers from the IFTTT ecosystem into three categories: public, private, and available. Triggers labelled as public contain information (e.g. new posts on reddit) that can be accessed directly from the Internet without any user authorization, and therefore we don’t consider them to be sensitive. For triggers labelled as private (e.g. new text messages), we consider their data to be sensitive, but except for a few exceptions the time when they happen is not. For triggers labelled as available (e.g. door unlocked), we consider both their data and their time to be sensitive information.






% \paragraph{In-scope of threat model.}
% As stated before our primary goal is to ensure the trigger-action platform (TAP)
% learns nothing about the trigger or action data. It should also not learn any
% sensitive constants embedded in the rule functions $\fone$ or $\ftwo$. TAP
% maintains the user OAuth tokens for secure communication between trigger and the
% action, so it learns the owner of the executed rule, and the corresponding
% trigger and action services, but it does not learn the function being evaluated
% in TAP.

% To meet the data privacy of the current TAPs we also ensure ..\rcnote{working here.}
% We do not want the action service (similarly, trigger service) to learn anything
% more about the trigger data (or action data) than what it already knows from the
% action data (or trigger data).


% Formally we model each of the services --- TS, AS, and TAP --- as honest but
% curious entities, who adheres to the said protocol but are inquisitive about
% other parties' data. Each entity is entrusted with a certain fraction of the
% data, and ideally they should not learn anything beyond what is revealed by
% their portion of the data.  We also assume that the parties do not collude.




% % We assume a strong attacker model: the attacker is the TAP, which means the
% % attackers not only can monitoring the network communications between the
% % platform and online services but also have access to the data stored inside the
% % platform. We will adopt a semi-honest model: the platform still executes the
% % rules correctly, but it is actively eavesdropping on the user data and might
% % leak the user data outside of the platform.

% \paragraph{Out-of-scope.}
% Since our goal is to provide confidentiality of sensitive user data, we do not
% prevent the case where a compromised TAP arbitrarily changes the rule semantics
% or refuses to execute the rule. In addition, we assume that online services for
% triggers and actions are not compromised. If they are compromised, the attackers
% can achieve the goal without interacting with the TAP.



%  LocalWords:  programmatically


==> design.tex <==
\section{Design of~\stap}
\label{sec:design}
%One of the goals while designing \stap was to ensure that TAP should continue to
%provide the level abstraction between TS and AS as it provides now. To make TAP
%oblivious of the trigger data $\dt$, we can encrypt the data with a key that is
%only available to the AS. Some types of trigger data, such as an images or media
%files, are never modified by (current) TAPs. For such data, simple encryption
%would suffice to provide confidentiality.  However, for other types of trigger
%data such as numbers of strings, using encryption would prevent computing any
%functions over it.

%We, therefore, use a combination of cryptographic schemes to enable secrecy of
%the trigger data.  % To do so,
% we have to redesign trigger-action platform from ground up. In this section we
% will detail the design of our \stap.
%We first describe the cryptographic schemes used in \stap, and then discuss design details.

% high level overview of our approach: we split trust and do GC

We use garbled
circuits~\cite{yao1986generate,yao2005design,bellare2012foundations} to design
our trigger-action platform, \name, so that TAP can compute a pre-defined set of
non-trivial functions over sensitive data without learning the trigger data, the
user-supplied constants, and the result of
computation. % At a high-level, our work is
% We % a set of protocols that
% use garbled circuits as a primitive. 

\begin{figure}[t!]
\centerline{\includegraphics[width=0.5\textwidth]{images/overview.png}}
\caption{Overview of \stap.}
\label{fig:arch_overview}
\end{figure}

\subsection{High-level design of \stap} A major difference between our work and
existing TAPs concerns the role of the client. Recall that the client is a
smartphone app or webapp that users program rules with. In current TAP design,
the client and the TAP itself is written by the same entity (e.g., IFTTT or
Zapier).  In \name, we require the client to be maintained by an entity
\textit{other} than the TAP provider. We envision a community of developers
building clients for our open \stap protocol. The app is possibly also
open-sourced and vetted for security by the community. % and
% then hosting them on various marketplaces (e.g., Android or Apple Store). 
% The
% app market model naturally results in a few well-built apps emerging to the
% top. For example, the Google Play store has hundreds of SSH client apps, with
% only a few being highly rated and downloaded. We see a similar situation with
% other open protocols such as Telnet, FTP, etc. Additionally, the open source
% community can independently vet open clients for security issues. Therefore, we
% envision a similar situation for the client in our setting.

With this added trust, we extend client functionality to generate garbled
circuits and the associated encoding/decoding information for user rules. The
encoding information is generated using a secret key shared between the client and
the trigger service, while the garbled circuits and decoding information are generated
through a customized protocol. The client encrypts the decoding information with
another secret key shared with the action service and sends it to the TAP along with the garbled circuits.

%First, like prior work, we take trust away from the trigger-action platform, and place it in the user's client. This is a smartphone or browser app that the user already trusts to not be malicious. In \name, we generate garbled circuits representing the computation over sensitive data inside the user's client. It then sends the circuit to the untrusted cloud-based TAP. It also sends the encoding information to the trigger service that enables it to convert its sensitive data to labels that a garbled circuit can consume. The client also sends decoding information to the action service so that it can learn the results of the garbled circuit evaluation. After performing these rule setup steps, the client is \emph{not needed} during rule execution. 

During rule execution, the TS will use encoding information to
convert plaintext data to labels, send those labels to the TAP, that uses the
garbled circuit to evaluate the function. Finally, the TAP sends the output
labels (along with the encrypted decoding information) to the AS which can decode the labels. \name also prevents the TAP from learning the result of the
predicate function $\fone$, as this can leak sensitive information as well.
We give the high-level view of the design in~\figref{fig:arch_overview}. 

After the system executes a rule, it deletes the used garbled circuit and associated encoding/decoding information. 
Thus, the client has to periodically
generate a set of garbled circuits and associated information and transmit those
to the TAP. This happens asynchronously from rule
execution. For example, the client can generate and transmit a batch of circuits
at night while the phone is being charged. 
Therefore, the client does \emph{not} need to be online during rule execution. 
Our evaluation demonstrates that this
overhead is less than an hour of streaming HD video (Section~\ref{sec:eval}).

% \name achieves security (we formally prove guarantees in
% Section~\ref{sec:security-analysis}) in the presence of a malicious circuit
% evaluator (i.e., TAP) that can arbitrarily deviate from the rule execution
% protocol. %because of our decentralized design that splits trust --- every user has
% their own trusted client that generates garbled circuits.

Next we discuss the cryptographic primitives we used for designing \name and go on to give the complete design.

\subsection{Used cryptographic primitives}\label{sec:crypto-tap}
We use a symmetric-key encryption scheme and a garbled circuit scheme to protect
sensitive user data.  Let $\H\Colon\zo^*\to\zo^\keylen$ be a cryptographic hash
function.
% Following our analysis of rules~\secref{sec:tap}, we
% found that some rules do not require any computation at TAP, beyond simple check
% of if the trigger fired. Providing confidentiality of such rules is easy by
% encrypting the trigger data, which TAP just forward to the AS. However, for a
% large fraction of rules, TAP performs some computation over the trigger
% data. Traditional encryption schemes would not allow such operations over the
% encrypted data.

% Therefore, we use two different types of encryption scheme to provide
% confidentiality of the trigger data. First, we use garbled circuit to protect
% the data that requires computation on the $\TAP$. Second we will use a
% symmetric-key encryption scheme to protect the data that does not require any
% computation on TAP. Below we briefly describe these two encryption schemes we
% will use while designing \stap.

\paragraph{Symmetric-key encryption scheme.} % In addition to the garbled circuit
% we will use symmetric encryption to hide data from TAP. 
Let $\ske = (\skegen, \skeenc, \skedec)$ be a semantically secure encryption
scheme. The key generation function $\skegen(1^\keylen)$ generates a
$\keylen$-bit uniformly random key $\key$; the randomized encryption scheme
$\skeenc$ takes a message $x\in\calX$ and the generated key $\key$ as input and
outputs a cipher text $\ctxt \getsr\skeenc(\key, x)$; and the deterministic
decryption function takes a cipher text and the key $\key$ as input and outputs a
message, $x \gets \skedec(\key, \ctxt)$, or $\bot$ (if decryption fails).

We use an authenticated encryption scheme
~\cite{bellare2000authenticated} for our implementation. Authenticated encryption schemes achieve the \textsf{IND-CCA} security guarantee that ensures both \textit{confidentiality} and  \textit{authenticity} of the plaintext.
\begin{comment}Semantic security ensures that no adversary (running time polynomial in
$\keylen$) can distinguish between the encryptions of two different messages (of
the same length). We expect the encryption scheme $\ske$ to also be
\emph{robust} and \emph{non-malleable}.  An encryption scheme is called
robust~\cite{abdalla2010} if the decryption fails --- outputs $\bot$ --- with
when a cipher text is decrypted with a wrong key. Non-malleability is a property
of the encryption scheme that ensures that without access to the key $\key$, no
adversary can forge or tamper with a cipher text such that it decrypts to a
valid plain text --- outputs anything other than $\bot$.  We will use
authenticated encryption with associated data
(AEAD)~\cite{bellare2000authenticated} to achieve all of these properties
simultaneously.
\end{comment}


% first introduced by
% Yao~\cite{yao1986generate} and later formalized as a primitive by Bellare et
% al.~\cite{bellare2012foundations}, 

\paragraph{Garbled circuits.} To enable secure function evaluation, we use
garbled circuits (GCs)~\cite{yao2005design,bellare2000authenticated}, a key cryptographic technique that allows computing a function without revealing the private inputs.
Following Bellare et al.'s~\cite{bellare2012foundations} notations, let a
garbling scheme $\G$ be a tuple of four functions $\G=(\Gb, \En, \Ev, \De)$. Let
the function to be garbled, without loss of generality, be
$f\Colon\zo^n\to \zo^m$, which is represented as a boolean circuit containing
only  AND ($\wedge$) and XOR ($\oplus$) gates.

% \begin{newitemize}
% \item
The \emph{garbling \ function} $(\Gb)$ takes a security parameter
  $1^\keylen$ and the function $f$ (represented as a boolean circuit) as input
  and outputs $(F, e, d)\getsr\Gb(1^\keylen, f)$. Here, $F$ is the
  \emph{garbled} version of the function $f$; $e$ and $d$ are the encoding and
  decoding information, respectively.  $\Gb$ is a randomized function.
  % \item
  The \emph{encoding \ function} $(\En)$ encodes an input $x\in\zo^n$
  using the encoding information $e$; $X\gets\En(e, x)$.
%\item
  The \emph{evaluation \ function} $(\Ev)$ enables evaluation of the circuit
  $F$ over the encoded input $X$; therefore $Y\gets\Ev(F, X)$.
  % \item
  Finally, the \emph{decoding \ function} $(\De)$ decodes the output of the
  evaluation; $y\gets\De(d, Y)$.
%\end{newitemize}

The correctness of a garbling scheme ensures that for all inputs $x$ if
$(F, e, d) \getsr \Gb(1^\keylen, f)$ then $\De(d, \Ev(F, \En(e, x))) = f(x)$.
We also mention here (informally) the relevant security definitions~\cite{bellare2012foundations} of GCs that we use (Assuming $f$ is public).
\begin{newitemize}
\item \emph{Message \ obliviousness.} Adversary learns nothing about $x$ or $y$
  (beyond what is known from $f$) given $(F,
  X)$ %leaks no information about $x$ or $y$
\item \emph{Input \ privacy.} Adversary learns nothing about $x$ beyond what is
  known from $y$.  given $(F, X, d)$
\item \emph{Execution \ authenticity.} % A garbling scheme is considered authentic
  % if given a garbled circuit $F$ and a 
  Given a garbled input $X$, it is hard to find $\tilde{Y}$ such that
  $\tilde{Y}\ne\Ev(F, X)$ and $\De(d, \tilde{Y})\ne\bot$.
\end{newitemize}

% To meet our security requirements specified in the threat model, we would use
% a garbling scheme that have these two security properties.



% \rcnote{Can we just borrow from emp-toolkit that their scheme provides
%   obliviousness and authenticity? and only prove the small delta that we have.}

% We present every operations in boolean circuit for garbling. This is
% straightforward for arithmetic operations, however, not so for string
% operations. Most of the string operations can be captured using a subset of
% regular expressions. We therefore created a simple engine to convert regular
% expression-based operations into boolean circuit. The details of our operation
% is given in~\appref{app:bool-regex}.

% From our analysis of rules in~\secref{sec:rules}, we found that arithmetic
% functions are not used in conjunction with arithmetic operations. While in
% theory, garbled circuit can be use to solve such mixed-operations, we found that
% our garbling scheme will become computationally and bandwidth-wise
% expensive. Therefore, currently, we don't support using both arithmetic and
% string operations in the same function. We leave for future studies to explore
% efficient ways to use the two operations in one function, if
% required. \rcnote{the language is quite loose.}

% \ef{discuss abstract model and how we derived it including the set of supported functions, then discuss concrete design, and finally show security arguments}

% % abstract model
% % concrete design:
% %  -- system-level design
% %  -- protocol design for numerics, string DFA
% % security arguments

\subsection{Architecture}\label{sec:arch}
% \ef{this should flow as: system architecture diagram plus explanation of each component, discuss an example rule and how it would execute. When we introcude the Trusted Client, we should motivate why this design choice is reasonable.}
% \figref{fig:arch} shows the architecture of \name.
We reuse the architecture of the existing trigger-action systems, but added some
extra functionalities to each component.  As before, $\stap$ has four
components: client's device ($\TC$), trigger service ($\TS$), action service
($\AS$), and a trigger-action platform ($\TAP$). % The main departure from a standard trigger-action system is that we designate the client to be trusted and separate from the cloud-based trigger-action platform.
As discussed earlier, we assume the client is trusted and refer to as trusted client $\TC$.   % it is built by an entity different from TAP.
% hereafter, we refer to the client as $\TC$. % and is trusted, and  envision that the trusted client is written by an entity separate from the TAP, and is similar to other open protocols like SSH or Telnet.

In \name, $\TC$ participates during the rule setup phase, and then periodically
generates and sends garbled circuits to $\TAP$. The trigger and action
services apply a shim over their API endpoints that transparently translates
between the encoded and decoded versions of their data. Instead of computing the
function over plaintext trigger data, $\TAP$ will evaluate the garbled circuit
over the encoded trigger data.

\paragraph{Rule setup (performed by the trusted client).}
The setup phase happens when the user installs a new rule in \name % the normal setup routine
% similar to current trigger-action systems.
using their client device \TC.  Similar to current TAPs, it connects a trigger
service $\TS$ with an action service $\AS$ by acquiring necessary OAuth tokens
from $\TS$ and $\AS$. In the push model of trigger-action systems, $\TAP$
generates a secret callback address for $\TS$ so that $\TS$ can actively
transmit trigger data.  The user also specifies the functions
($\fone$ and $\ftwo$) to be evaluated at $\TAP$ via a click-through user
interface and, if required, the constant parameters ($\cone$ and $\ctwo$).
Every rule is assigned with a rule id.

Additionally, in our new design, \TC generates and stores two random values
$\sects, \secas \in \zo^\keylen$, which are secret keys to be shared with \TS
and \AS respectively. Furthermore, \TC, \TS, and \AS creates a new variable
$j$, which will be used as the circuit id and is initialized to 0.
% Next, \name additionally requires \TC to generate and store two random strings $\sects, \secas \in \zo^\keylen$, which are secret keys to be shared with \TS and \AS, respectively, and a random integer $j$, which is used as the circuit id. $\sects$ and $j$ are sent to \TS while $\secas$ and $j$ are sent to \AS during this setup phase.
\rcnote{Why do you have to generate/send the circuit id $j$ during setup? Do you mean rule-id? I commented it out; if necessary you can uncomment it back. }
\yc{$j$ here refers to the initial circuit id, which will get incremented after each rule execution}

The rule id, callback addresses, the OAuth tokens are uploaded to $\TS$, $\AS$,
and $\TAP$ accordingly as it is done in current trigger-action systems. However,
the functions, the constants, and the secret keys $\sects$ and $\secas$ are
stored locally on~$\TC$. The secret $\sects$ is shared with $\TS$, and $\secas$ is shared with $\AS$. 


\begin{figure}[t]
\centerline{\includegraphics[width=0.4\textwidth]{images/rule_setup_execution_11.png}}
\caption{Diagram showing the high-level architecture of \stap. The client $\TC$ garbles the circuits and forwards them to \TS,\TAP, and \AS. During rule execution we don't need the client to be online.}
\label{fig:arch}
\end{figure}

\begin{figure}[h]
  \centering\gamesfontsize
  \hfpagess{0.21}{0.225}{
    \underline{\textsf{CktGarbling}($(f, \const), (j, \sects, \secas)$)}:\\[2pt]
    $\eis \gets \H(\sects \concat j \| 0) $\\
    $\eir \gets \H(\sects \concat j \concat 1) \lor 0^{\keylen-1}1 $\\
    $\key \gets \H(\sects \concat j \concat 2) $\\
    % $\ei\gets(\eis,\eir)$\\
    $(F, \di, h) \gets \Gb'\left((\eis,\eir), f\right)$\\
    % $(F, \wlabel^{w_0}_0, \ldots, \wlabel^{w_m}_0) \gets \Gb'(f, \ei)$\\
    % $d \gets (\textsf{lsb}(\wlabel^{w_1}_0), \ldots, \textsf{lsb}(\wlabel^{w_m}_0))$\\
    % $h \gets \H(\wlabel^{w_1}_0 \concat \ldots \concat \wlabel^{w_m}_0)$\\
    $\encd \getsr \skeenc(L^{w_0}_1 \oplus \secas, (j, k, \eir, d, h)) $\\
    $C \gets \En(\ei, \const)$\\
    % $j \gets j + 1$\\
    Return $j, F, C, \encd$\\[2pt]

    \underline{\textsf{TriggerExec}$\left((\dt, \payload), (\sects, j)\right)$:}\\[2pt]
    $\eis \gets \H(\sects \concat j \concat 0)$\\
    $\eir \gets \H(\sects \concat j \concat 1) \lor 0^{\keylen-1}1  $\\
    $\key \gets \H(\sects \concat j \concat 2) $\\
    % $\ei\gets(\eis,\eir)$\\
    $\LT \gets \En\left((\eis,\eir), \dt\right)$\\
    $t \gets \textsf{CurrentTime()} $\\
    $ct \getsr \skeenc(k, (t, \payload))$\\
    $\return j, \LT, ct$
   }
  {
    \underline{\textsf{PlatformExec}$\left((j,X,ct), (F,C,\encd)\right)$:}\\[2pt]
    $Y \gets \Ev(F, (\LT, C))$\\
    $\return j, \LA, ct,\encd$\\[2pt]
    
    
    \underline{\textsf{ActionExec}$\left((j, \LA, ct,\encd), \,\secas\right)$:}\\[2pt]
    Parse $\LA$ as $(\wlabel^{w_0}, \wlabel^{w_1}, \ldots, \wlabel^{w_m})$\\
    $z\gets \skedec(\wlabel^{w_0} \oplus \secas, \encd)$\\
    If $z = \bot$ then \ $\return \bot$\\
    $(j', k, \eir, d, h) \gets z$\\
    $y \gets \De\left(d, \LA\right)$\\
    $g\gets \bot$\\
    For $i\gets 1$ to $m$ do\\
    \mytab If $y_i = \false\;$ then $\;g\gets g\concat\wlabel^{w_i}$ \\
    \mytab Else $\;g\gets g \concat (\wlabel^{w_i}\oplus\eir)$\\
    % $h' \gets \H\left( (\wlabel^{w_1} \oplus y_1 \eir) \| \ldots \| (\wlabel^{w_m} \oplus y_m \eir) \right)$\\
    $h' \gets \H(g)$\\
    $(t, \payload) \gets \skedec(k, ct)$\\
    $t'\gets \textsf{CurrentTime}()$\\
    If $t'> t+\delay$ or $h \ne h'$ or $j \ne j'$ then\\
    $\mytab\return~\bot$\\
    $\return y, \payload$
  }
  
  \caption{Circuit generation and rule execution protocols for $\stap$.
    $\wlabel^{w_0}_1$ denotes the $\true$ label chosen of the first output wire $w_0$;
    $\delay$ is a threshold parameter used to ensure the freshness of a
    trigger. The \textsf{CircuitGarbling} is run by the client $\TC$
    asynchronously of the actual rule execution.  The remaining three functions
    are run by \TS, \TAP, and \AS during rule execution.}
  \label{fig:algo}
\end{figure}



\paragraph{Circuit garbling (performed on the trusted client).} 
% At a high level, \TC periodically use the secret keys to generate a number of garbled circuits for the
% user-specified function, along with associated encoding and decoding information. 
% The garbled circuit distribute them to \TAP. 
% The garbled circuit, $\{j, F_j\}$ along with the labels for the constants are sent
% to the $\TAP$. The encoding information $\{j, e_j\}$ is sent to the $\TS$, and
% the decoding information to $\AS$.
%From this section onward,
We will represent the user-specified functions ($\fone$ and $\ftwo$) as Boolean circuits consisting of  XOR~($\oplus$) and AND ($\wedge$)
gates only. Also, without loss of generality, we assume that the domains of $\fone$ and $\ftwo$ are the
same, and the constants and trigger data are all from $\zo^n$, that is
$\fone\Colon\zo^n\times\zo^n\to\zo$ and
$\ftwo\Colon\zo^n\times\zo^n\to\zo^m$. We further simplify the notations by
concatenating the circuits of the two functions together and reusing some input
wires for the trigger data. We also let $\const=(\cone, \ctwo) \in\zo^{2n}$.
So, let $f\Colon\zo^n\times\zo^{2n}\to\zo^{m+1}$, such that
$f(\dt, \const) = \fone(x, \cone)\|\ftwo(x, \ctwo)$. We denote $f$ as the
function we garble and evaluate at the $\TAP$ with constants $\const$. We only mention $\fone$ and $\ftwo$ or $\cone$ and $\ctwo$ when required.


% We modify the standard garbled circuit primitive to fit our security
% requirements. % We discuss the modifications next.



\rcnote{Up to here. We should talk about generic garbled circuit first and then show our modification.}
\paragraph{\textnormal{\emph{Encoding Blob.}}} The client $\TC$ first generates two bitstrings $(\eis, \eir) \in \zo^{2\keylen}$ using the hash value of $\sects \concat j$. The value $\eir$ is a global offset used by free XOR optimization~\cite{kolesnikov2008improved}, and $\eis$ is the seed for generating
random labels (as described below); together they form the encoding information
$\ei=(\eis, \eir)$ for garbled circuit protocols. 
\TC also generates another bitstring $\key \in \zo^\keylen$, which is the key to
encrypt trigger payload data~$\payload$. We refer $(\ei, \key)$ as the encoding blob.

\paragraph{\textnormal{\emph{Garbled Circuit.}}} To garble a circuit, each wire $w$ in the circuit needs two random labels
$\wlabel_1^w$ and $\wlabel^w_0$ --- representing the $\true$ and $\false$
values. We
will use a pseudo random function (PRF), $\mathcal{F}$ of output bit size $\kappa$ to assign the
labels for input wires.

For each input wire $w$ in the boolean circuit of $f$, the labels
are generated as $\wlabel^w_0 = \mathcal{F}(\eis, w)$ and
$\wlabel^w_1 = \wlabel^w_0\oplus \eir$. (We assume there is an unambiguous way
to represent wire index $w$ as a fixed-length bitstring).  
Given the encoding information $\ei$ and along with wire index information, the
encoding function $\En(e,\cdot)$ takes as input a bitstring $\dt$ and outputs a
sequence of labels corresponding to the input wires.  % Note the encoding
% information $\ei$ () is sufficient to compute the labels for $\dt$.
% The least significant bit of $R$ is always
% set to $1$.\rcnote{We might not need this modification as we send the whole
%   label.} $\ei_\dt$ and $\ei_\const$ will be used as a seed to the PRF to
% generate labels. 

% We set labels for each wire $w$ as $\wlabel^w_0 = \H(\eis\|w)$. % For the
% % input wires corresponding to the constants, we will use different seed $\c$,
% % we use $\wlabel_0^w = \H(e_c\|w)$.
% For each wire $w$, we set $\wlabel_1^w =
% R\oplus\wlabel_0^w$.  % Let $C_1$ and $C_2$ be the sets of labels
% % for the client's constants $\cone$ and~$\ctwo$.

Next, we can start to garble the gates and compute the labels for non-input wires. We refer the reader
to~\cite{zahur2015two} for details on the garbling scheme. 
However, different from the standard garbling function, we add two modifications: (1) The encoding information is pre-computed and fed into the function, instead of being randomly generated inside the function; (2) the $\false$ labels of all output wires are returned, instead of just the decoding information, in order to construct the decoding blob. We denote this customized garbling function as $\Gb'$.

% We use $\Gb'$ to denote the non-standard garbling function that takes a function $f$ (represented as a
% boolean circuit) and required encoding information $e$ and returns a garbled
% version of $f$ along with the $\false$ labels of all output wires.  
% 


\newcommand{\hwlabel}{h}
\paragraph{\textnormal{\emph{Decoding Blob.}}} The decoding blob first includes 
the garbled circuit's decoding information $d$, which is used to
translate the labels of output wires back to bits. Let the output wires for the function $f$ be
$(w_0, w_1, \ldots, w_m)$, where $w_0$ corresponds to the output wire of $\fone$, and
the remaining $m$ wires for the function~$\ftwo$. As the standard practice in
optimized semi-honest garble circuits protocols, $d$ contains the least significant bits of the $\false$ label of each output wire ($\textsf{lsb}(\wlabel^{w_0}_0), \ldots, \textsf{lsb}(\wlabel^{w_m}_0)$). We slightly modify $d$ by removing its first bit ($\textsf{lsb}(\wlabel^{w_0}_0)$) (since the decoding of $w_0$ is covered by a encryption layer described later in this section).

However, using $d$ alone cannot achieve our integrity goal against a malicious \TAP that sends forged output labels --- we need another mechanism to ensure the authenticity of labels.
Therefore, we compute the hash of the concatenation of output labels and add this hash value, denoted by $h$, to our decoding blob.
Specifically, the $\false$ labels of 
all output wires are concatenated and then hashed, i.e.$h = \H(\wlabel^{w_1}_0 \concat \ldots \concat \wlabel^{w_m}_0)$.
% Note in this way the $\TC$ does \emph{not}
% reveal any information about the label of wire $w_0$ (output of $\fone$) to the $\AS$.

We also append the payload key $k$, the XOR offset $\eir$, and the current circuit id $j$ to the decoding blob, all of which are required by \AS during the execution step. 

Next, we encrypt the decoding blob with two keys: $\secas$, which is the secret key shared with \AS, and $\wlabel_1^{w_0}$, which is the $\true$ label of $\fone$'s output wire $w_0$. This encryption ensures that \TAP will never learn the decoding blob (since it does not have $\secas$) while \AS
will only be able to learn the decoding blob when the predicate $\fone$ is evaluated true (otherwise it will receive $\wlabel_0^{w_0}$ instead of $\wlabel_1^{w_0}$). We denote this encrypted decoding blob as $\encd$.

Finally, \TC computes the labels for the user-provided constants $C \gets \En(\ei,\const)$ and sends $(j, F, C,\encd)$ to the \TAP. Before garbling the next circuit, 
\TC increments the circuit id $j$ by 1.
  
% When \AS
% receives a tuple of labels $(\wlabel^{w_1},\ldots,\wlabel^{w_m})$ from the \TAP after circuit evaluation, it computes $\wlabel^{w_i}_0 = \wlabel^{w_i}_{y_i} \oplus y_i \eir$ for each output wire after getting $y_i$ from the decoding procedure and the hash of
% their concatenation. If the new hash does
% not equal to the one received from \TC, the decoding procedure will fail, which allows us to
% catch if a malicious TAP lying about the output of the function $f$.


%the value of the output wire $w_i$ is set to $b$ if
%$\exists\ b\in\zo,\,\H(\wlabel^{w_i}) = \H(\wlabel^{w_i}_b)$, and $\bot$,
%otherwise.  



%Also, the
%$hashing protects the global XOR-offset $\eir$ from the action service.  



% Finally, we don't want \name to learn about the decoding information, nor should the action service  when
% output of $\fone$ is $\false$. % is the first wire $w_0$ is set to zero.
% We, therefore, encrypt the decoding information $d$ with the $\true$ label of
% the output wire $w_0$ (i.e., $\wlabel_1^{w_0}$) and \AS's secret string: the client computes
% $\encd\getsr\skeenc(\wlabel^{w_0}_1 \oplus \secas, (d, k, h, \eir, j))$. The encryption ensures 
% \name will never learn any results of its output
% while \AS
% will only be able to learn the result of $\ftwo$ when the predicate $\fone$ is
% true.

%would not learn anything about the decoding information without receiving the
%correct $\true$ label $\wlabel_1^{w_0}$ from \TAP. 

% Note
% However, the way
% labels are generated, we cannot send $\{L^w_0, L^w_1\}$ for each output wire
% $w$; else the trigger service will learn the XOR-offset $R = L^w_0\oplus L^w_1$,
% which enables inquisitive $\TS$ to learn about the decoding information $d$,
% even when the the first bit of the output of $f$ (or $\fone$ evaluates to
% $\false$).



% First, the client generates four
% random strings, $\ei_\dt, \ei_c, R, k \in \{0,1\}^\keylen$:
% \begin{itemize}
% 	\item $\ei_\dt$ and $\ei_c$ are the seeds of the PRG: $\{ 0, 1 \}^\keylen \to \{ 0, 1 \}^l $, where $l \gg \keylen$.
% 	\item $R$ is the free-XOR offset common to all wires. To enable the point-and-permute technique, the least significant (last) bit of $R$ is manually set to 1.
% 	\item $k$ is the key to the symmetric-key encryption scheme.
% \end{itemize}

% Then for each input wire that belongs to the trigger data $\dt$, we use $\PRG(\ei_\dt)$ to generate its FALSE label, i.e. the $i$-th input wire will use the $ik$-th to $i(k+1)$-th bits from the output of PRG as its FALSE label. The TRUE label is computed by xor-ing the FALSE label with $R$. \yc{Describe this in mathematical terms?} Similarly, the labels for the input wires that belongs to $\cone$ or $\ctwo$ are generated using $\PRG(\ei_c)$.

% Next, the garbling protocol $\Gb(1^\keylen, (\fone, \ftwo))$ is executed, which will produce
% \begin{itemize}
% 	\item The TRUE and FALSE labels for each wire in the circuit,
% 	\item $\Fone$ and $\Ftwo$, the garbled version of $\fone$ and $\ftwo$.
% \end{itemize}

% Finally, \TC creates a unique identifier $j$ for this execution and sends
% \begin{itemize}
% 	\item $j, e^{(j)}$ to \TS, where $e^{(j)} \gets (\ei_\dt, R, k)$;
% 	\item $j, F^{(j)}, C^{(j)}$ to \TAP, where $F^{(j)} \gets (\Fone, \Ftwo)$ and $C^{(j)} \gets (C_1, C_2)$, which are the labels corresponding to $\cone, \ctwo$;
% 	\item $j, d^{(j)}$ to \AS, where
% 	\begin{itemize}
% 	    \item $d^{(j)} \gets (d_{f_1}, \Enc_{L_1^p}(d_{f_2}, k)) $,
% 		\item $d_{f_1} = \textsf{lsb}(L_0^p)$ is the least significant bit of the FALSE label for $f_1$'s output wire,
% 		\item $d_{f_2}$ contains the hashes (computed via hash function $H$) of the TRUE and FALSE labels for every $f_2$'s output wire,
% 		\item $L_1^p$ is the TRUE label for $f_1$'s output wire.
% 	\end{itemize}
 
% \end{itemize}
% \yc{check notation consistency}


% We extend this functionality of the trusted client to periodically generate the
% garbled circuits and associated encoding and decoding information and distribute
% them to the TS, TAP, and AS. We believe this periodic engagement is practical,
% and as we show via our experiments, computationally feasible for average
% cellphones or computers.  \rcnote{Check with DTAP paper to find more plausible
%   argument of the trusted client.}

\paragraph{Rule execution (does not involve client).}
When a trigger event happens, \TS sends the event data to the callback URL provided by \TAP. \TAP evaluates the function $f$ in an oblivious manner and forwards the output to the action service. The three functions executed by \TS, \TAP, and \AS is noted in~\figref{fig:algo}. 
For simplicity, we omit the standard OAuth authorization steps.

$\TS$ retrieves
$(\sects, j)$ from its storage, and performs the \textsf{TriggerExec} function on
the trigger data $(\dt, \payload)$. It generates the encoding blob similar to the 
client's \textsf{CktGarbling} function. Then part of the data, $\dt$, is encoded as $X$
using the function $\En(\ei,\cdot)$, while the payload $\payload$ is encrypted
using the key $\key$. \TS also appends a timestamp $\ts$ to the payload data, that
will be used later to determine the freshness of the trigger event by the action
service. Let $ct\getsr\skeenc(k, (t, \payload))$. \TS forwards $(j, X, ct)$ to
TAP. Similar to \TC, \TS also increments $j$ by 1 at the end.

\TAP, on receiving a trigger message $(j, X, ct)$, retrieves the corresponding garbled circuit $F$, encoded constants $C$, and the encrypted decoding blob $\encd$ using the circuit id $j$. \TAP applies the garble circuit evaluation function $\Ev$ on $X$ and forwards the tuple $(j, Y, ct, \encd)$ to the \AS. 

\AS first verifies the circuit id $j$ it receives from \name is greater than any circuit id it has
seen previously, and then executes the function \textsf{ActionExec} using the data received
from \TAP and $\secas$ as parameters. \AS can only decrypt $\encd$ to obtain the decoding blob when $\fone$ is evaluated $\true$ (i.e.  $\wlabel^{w_0} = \wlabel_1^{w_0}$); otherwise the function will fail and output $\bot$. The function may also fail if the message
from \TAP is malformed or stale. The authenticity of the message is determined by converting each received label (except the first one) to the corresponding $\false$ label and then comparing the new hash with the hash embedded in the decoding blob, while the staleness is checked through the timestamp $t$ and circuit id $j$. The final output of \textsf{ActionExec}, other than $\bot$, is fed to the
action API.

% Each service uses $j$ to synchronize the garbled circuits and associated
% information to use. Therefore, if a service does not find a valid database entry
% for a circuit id $j$, the associated message is silently dropped. Also, after a
% circuit id is used, each service is supposed to delete the associated
% information from their database. \TS will never reuse a circuit for encoding
% its trigger data. This provides forward secrecy to the system in case the
% attacker compromises both \TS and \AS.  The client $\TC$ periodically generates a number of circuits and sends them to \TS, \AS, and \TAP. 


\subsection{Converting functions to boolean circuits}\label{sec:boolfunc}
% \subsection{Converting string operations to garbled circuits} 
% \label{sec:gc-ops-string}
While in theory any computable function can be converted into boolean circuits,
and therefore can be computed using garbled circuits, in practice
they can be very expensive. For example, EMP toolkit supports boolean and
arithmetic operations natively, but does not support string operations because input dependent branching is disallowed in garbled circuit
evaluation (otherwise it will indeed reveal the input data).
%emulating strings
%operations over array of characters is also difficult.  
We therefore devise a
novel method to convert string operations requiring regular expressions into
boolean circuits that are efficient for GCs.

\paragraph{Converting DFAs into Garbled Circuits.}  Based on our analysis of the rules the commercial TAPs currently support (Section \ref{sec:supported-functions}), we observe that a large fraction of them are string operations that involve matching and substring extraction/replacement. Regular expressions can be converted into deterministic finite automaton (DFA) for easy evaluation.
Mohassel et al.~\cite{mohassel2012efficient} introduced an oblivious deterministic finite automata (Obliv-DFA) approach to match regular expressions in an SMC setting. However, their approach % requires the supplier of the input string to eventually evaluate the output, which contradicts our security requirement. In addition, the output of Obliv-DFA \ef{cannot be computed with other wires in the circuit} nor can it be
cannot be easily extended to support substring extractions and replacements.

Therefore, we implement a purely circuit-based approach to efficiently match a
DFA with an input string and support substring extractions and replacements. By
converting DFA matching to a Boolean circuit, we keep our existing garbled
circuit infrastructure, and retain the same security properties.

We describe the details of how to convert DFAs into Boolean circuits and how to extend to that to perform substring replacement and extraction in~\appref{app:regex}. We assume the input string is of fixed length and \TS unambiguously pads the string if the string is smaller.

For string replacement, we use our boolean circuit to replace the string with special symbols where the source pattern matches, and \AS replaces them with the replacement string. The replacement string is encrypted with the hash of the labels for the special symbol, so that \AS can only learn about the replacement string if there exists such a replacement. 
% In \secref{sec:arch}, we refer $\fone$ and $\ftwo$ as boolean circuits of fixed
% input and output sizes, instead of generic functions. While certain operations
% are quite straight forward to evaluate in garbled circuit (GC), some are
% not. For example, supporting boolean and arithmetic operations is quite straight
% forward. However, string operations, such as the one involve regular expressions
% (e.g., \texttt{extract\_phone}) is not efficiently handled by standard GCs.


\paragraph{Supported Functions.} 
By incorporating the above techniques, we can use garbled circuit to compute
practically all functions listed in~\figref{fig:functions} with three exceptions
(\texttt{format}, \texttt{strip\_html}, and \texttt{html2markdown}). We sketch
the implementation details for each supported function in~\appref{app:func-impl}. Based on our Zapier dataset collected in \secref{sec:supported-functions}, this
set of operations enables \name to support 93.4\% of the function-dependent
rules published on Zapier.

It is possible to convert the remaining three unsupported functions to boolean circuit, as well, but the resulting circuit will be very large (for example, we need to build a full-blown parser to find HTML tags). 

%In addition, we argue that these functions are only used for formatting, and do not add, remove or transform any sensitive information in their outputs. Therefore, we can choose to run them in \AS after the plaintext output is obtained and still retain our security goals. 


%Standard garbled circuits efficiently support boolean and arithmetic operations. Unfortunately, string operations can become inefficient with current frameworks because they will be broken down into very large circuits. Thus, Mohassel et al. introduced an efficient deterministic finite automaton (DFA) approach to support string operations that can be expressed using regular expression (e.g., pattern matching)~\cite{mohassel2010}. However, this approach does not meet our requirements because the party who holds the secret data must evaluate the DFA circuit. In our setting, the \TS holds the secret data. As discussed in Section~\ref{sec:towards}, this puts undue burden on the \TS and breaks the abstraction between \TS, \TAP, and \AS. However, we take inspiration from this approach and build an efficient scheme that converts a DFA into garbled circuits using a custom state encoding scheme. We go beyond regular expressions and also introduce techniques to perform substring extraction and replacement. We discuss our approach to matching regular expressions with garbled circuits next. Appendix~\ref{app:regex-extract} contains a discussion of how we extend this protocol to perform extraction and replacement.

% \subsubsection{Boolean and Numeric} 
% Existing secure multi-party computation frameworks like EMP toolkit~\cite{emp-toolkit} support boolean and integer or float operations efficiently. We use this support without any modifications.

% \paragraph{Input and output representations.} 
% If a field in the trigger data is a string, we require the \TS to first pad it to 
% a fixed length by appending some predetermined padding characters, as the length of the string may leak the actual content in the string when the input space is small. Then the string is encoded into a fixed-length bitstring $\vecx = (x_1,\ldots,x_n)$ where $x_i\in\zo$ before feed into the encoding function $\En$. Similarly, if an output field is a string, its size should also be fixed to some predetermined length. Therefore, 
% it is the duty of \AS to remove the padding characters after it retrieves the plaintext output.


% \paragraph{Converting DFAs into circuits.}

% We give a description of our approach below. A more concrete explanation on how to support substring extraction and replacement is presented in Appendix \ref{app:bool-regex}.
% Let $\dfa$ be a DFA, defined as a five-tuple,
% $\dfa = (\states, \alphabet, \trans, \State_0, \finalstates)$, where $\states$
% is the set of states, $\alphabet$ is the set of alphabets, $\State_0$ is the
% initial state, and $\finalstates$ is the final state. The transition function
% $\trans$ takes a state and an alphabet and returns the next state; therefore,
% $\trans\Colon\states\times\alphabet\to\states$.  As every string is a
% bitstring, we have $\alphabet=\zo$. Let $\nstates = |\states|$ be total number of states. Without loss of generality, we assume $\states = \mathbb{Z}_q  = \{1, \dots, q\}$.

% Let $\transstring$ be a function that takes a string as input and outputs the
% final state of the DFA after consuming the whole string starting from the state
% $\state_0$, %
% \bnm \transstring(\vecx) = \trans(\ldots\trans(\trans(\state_0,
% x_1),x_2),\ldots, x_n)  \enm If $\transstring(\vecx)\in\finalstates$, then
% $\vecx$ is accepted by the DFA, which means the string matches the regular
% expression.

% We encode each state into a bit-vector of size $\nstates$ using one-hot encoding. 
% We use $\State$ to denote the encoding of a state $\state \in \states$, and $\State^j$ represents the $j$-the bit of $\State$, where $\State_0^s = 1$ and $\State^j = 0$ for any $j \ne s$. 
% Therefore, the output of the DFA becomes 
% \bnm \Transstring(\vecx) = \Trans(\ldots\Trans(\Trans(\State_0,
% x_1),x_2),\ldots, x_n)  \enm
% where $\Trans$ is the transition function that operates on the encoded states.

% We also define two sets for each state $s$, $P_0^\state$ and $P_1^\state$, where 
% \bnm P_b^s = \{i\suchthat\trans(i,b) = j\} \enm for $b\in\zo$.


% %We will now specify the new transition function $\Delta$ is represented as a boolean circuit. 
% We now discuss how we represent the transition function as a boolean circuit, suitable for use with any standard frameworks that support free XOR optimizations. Let
% $T = \Trans(S, x)$. We can observe that $T^j=1$ if and only if either $x=1$ and $\exists i \in P_1^j, S^i=1$, or  $x=0$ and $\exists i \in P_0^j, S^i=1$. That is to say,
% \bnm T^j  = (x\wedge\bigvee_{i\in P^j_1}S^i) \vee (\neg x\wedge\bigvee_{i\in P^j_0}S^i)  = (x\wedge\bigvee_{i\in P^j_1}S^i) \oplus (\neg x\wedge\bigvee_{i\in P^j_0}S^i)  \enm
% % The second equality follows from the identity that $(a\wedge b)\vee(\neg a \wedge c) = 
% % (a\wedge b)\oplus(\neg a \wedge c)$, for any bit variables $a, b, c$.  
% Because only one of the $S^i$ will be 1 at any time, therefore the inner OR gates can also be replaced with XOR:
% \bnm T^j  = (x\wedge\bigoplus_{i\in P^j_1}S^i) \oplus (\neg x\wedge\bigoplus_{i\in P^j_0}S^i), \; \text{ for } 1\le j\le q.\enm
% Therefore, each bit in $T$ requires at most $2$ AND gates to compute (assuming XOR gates can be computed without any garbling cost). To run $\dfa$ over a string of length $n$, we need to apply $\Trans$ $n$ times, and the resulting circuit contains no more than $2n\nstates$ AND gates.

% Finally, to check if the final state is accepted by $\dfa$, simply computing $\bigoplus\limits_{j\in\finalstates}S_n^j$ is sufficient.

%We omit the details of how to convert a regular expression into a DFA; the
%reader can refer to~\cite{chang1992regular} on how to so efficiently. 

% We currently support a subset of regular expressions. On restriction that we require is there should not be any overlapping matching substrings: once the DFA reaches an accepting state, no further matching should be possible. This can be achieved by having a 
% \todo{Or any manual modification we have done. This restriction is only applied to the second replacement protocol.}


% \paragraph{Representing $\trans$ as a boolean circuit.}
% We represent each state as an one-hot encoding into a bit-vector of size
% $\nstates$, where $\state^j$ represents the $j$-the bit of the state $\state$.
% Without loss of generality, let assume $\state_0^j = 1$ for $j=1$, and
% $\state_0^j = 0$ for $1<j\le \nstates$. We note that exactly one location in the
% bit-vector is one for any state.  We also crate two sets for each state $j$, $P_0^j$ and $P_1^j$, where $P_b^j = \{i\suchthat\trans(i,b) = j\}$ for $b\in\zo$.


% We will now specify the transition function as a boolean circuit. Let
% $t = \trans(s, x)$. we claim that $t^j=1$ if and only if either $x=1$ and $\exists i\in P_1^j, s^i=1$, or  $x=0$ and $\exists i\in P_0^j, s^i=1$. That is to say,
% \bnm t^j  = (x\wedge\bigvee_{i\in P^j_1}s^i) \vee (\neg x\wedge\bigvee_{i\in P^j_0}s^i)  = (x\wedge\bigvee_{i\in P^j_1}s^i) \oplus (\neg x\wedge\bigvee_{i\in P^j_0}s^i)  \enm
% The second equality follows from the identity that $(a\wedge b)\vee(\neg a \wedge c) = 
% (a\wedge b)\oplus(\neg a \wedge c)$, for all bit variables $a, b, c$.  Also, because only one of the $s^i$ will be 1 at any time, there fore the inner Or gates can be replaced with XOR.
% \bnm t^j  = (x\wedge\bigoplus_{i\in P^j_1}s^i) \oplus (\neg x\wedge\bigoplus_{i\in P^j_0}s^i), \; \text{ for } 1\le j\le n\enm

% We can apply the modified boolean transition function $\trans$  to compute the final state $s_n = \transstring(\vecx)$, and to see if the final state is accepting or not we simply check if $\bigoplus\limits_{j\in\finalstates}s_n^j$ is 1 or not.
% This conversion ensures more number of XOR gates, which are more efficient to garble than AND gates.



% \paragraph{Garbled circuit size.} Each output bit of $\Trans$ requires at most $\nstates$ XOR gates and $2$ AND gates to compute. Therefore, each computation of $\Trans(\State, x)$ will take $\nstates^2$ XOR gates, and $2\nstates$ AND gates. Assuming the free XOR technique is applied, running DFA over a string of length $n$ will require the size of garbled circuit to be $\bigO(n\nstates)$.



% The message contains trigger data to describe the event. However, this doesn’t necessarily indicate the action will also be performed, since the user might add some additional checks on the trigger data. For example:

% \begin{itemize}
%     \item When the trigger is ``new SMS received", the rule might have some condition checks on the message text, such as whether it contains the word ``alert".
%     \item When the trigger is some time-sensitive condition such as ``the kid leave home", the rule might also add additional conditions such as ``which kid".
% \end{itemize}

% The execution diagram is shown in Fig \ref{exec_push} and the protocols for each party is described below:


% \paragraph{Trigger Service (\TS).} Once \TS has the trigger data $\dt$ and trigger payload $\payload$ ready, it selects a $j$ that has not been selected by previous executions and sets $(\ei_\dt, R, k) \gets e^{(j)}$. \TS executes the encoding protocol $$\LT \gets \En(\ei_\dt, \dt)$$ where $\LT$ is the labels of trigger data $\dt$ (similar to \TC's label generation procedure).

% Then, \TS records the current timestamp $t$ and computes $\Enc_k((j, t, \payload))$ using a symmetric-key encryption scheme. Finally, \TS sends $j$, $\LT$, and $\Enc_k((j, t, \payload))$ to \TAP. 


% \paragraph{Trigger-Action Platform (\TAP).} After receiving $j$, $\LT$, and $\Enc_k((j, t, \payload))$ from \TS, \TAP sets $(\Fone, \Ftwo) \gets F^{(j)}$ and $(C_1, C_2) \gets C^{(j)}$ and executes two evaluation protocols $$P \gets \Ev(\Fone, (\LT, C_1))$$ and $$Y \gets \Ev(\Ftwo, (\LT, C_2)),$$ where $P$ is the label of the predicate bit and $\LA$ is the labels of action data.

% Finally, \TAP passes $j, P, Y,$ and $\Enc_k((j, t, \payload))$ to \AS.

% \paragraph{Action Service (\AS).} After receiving $j$, $P$, $Y$, and $\Enc_k((j, t, \payload))$ from \TAP, \AS sets $(d_{f_1}, \Enc_{L_1^p}(d_{f_2}, k)) \gets d^{(j)}$. \AS first executes a decoding protocol
% $$ p \gets \De(d_{f_1}, P). $$

% If $p = 0$, \AS ignores the rest of the message and terminates the protocol. If $p = 1$, then $P = L_1^p$ and thus \AS can get $$(d_{f_2}, k) \gets \Dec_P(\Enc_{L_1^p}(d_{f_2}, k)).$$

% A second pair of decoding and decryption protocols is then executed to compute the action data $y$ and the payload $\payload$:
% $$ y \gets \De_H(d_{f_2}, Y) $$
% $$ (j', t', \payload) \gets \Dec_k(\Enc_k((j, t, \payload))) $$

% Finally, to ensure the integrity of the message, \AS needs to check if the following two conditions hold:
% \begin{itemize}
%     \item The unique identifier $j$ sent by \TAP equals to the unique identifier $j'$ selected by \TS,
%     \item $t - t' < \varepsilon$, where $t$ is the timestamp when the message is received by \AS and $\varepsilon$ is some predefined threshold.
% \end{itemize}

% \yc{Probably should use some algorithm boxes to represent the above protocols}




% \begin{figure*}[t!]
% \centerline{\includegraphics[width=\textwidth]{images/rule_setup_execution.png}}
% \caption{Rule execution Phase for pushing model.}
% \rcnote{Update the two figures to be consistent with the variables we are using in the text. Add a trusted client in this picture, thereby we can remove~\figref{setup}. Also make it compact to save some space.}
% \label{exec_push}
% \end{figure*}



% \begin{figure*}[t!]
% \centerline{\includegraphics[width=\textwidth]{images/rule_setup_execution.png}}
% \caption{Rule execution Phase for pushing model.}
% \rcnote{Update the two figures to be consistent with the variables we are using in the text. Add a trusted client in this picture, thereby we can remove~\figref{setup}. Also make it compact to save some space.}
% \label{exec_push}
% \end{figure*}

% \input{images/tap-image}
% \begin{figure*}[t!]
% \centerline{\includegraphics[width=\textwidth]{images/rule_setup.png}}
% \caption{Rule Set-up Phase. $key_1$ refers to a set of encryption information, $params$ is the parameters passed to the trigger API, $i_1, ...$ are indices of the fields in trigger data that the rule function needs to apply some operations on (data that needs to be encrypted to MPC labels), and  $j_1, ...$ are indices of the fields that are directly sent to action service (data that can be encrypted using any standard encryption techniques). Similarly, $key_1$ refers to a set of decryption information, and $k_1, ...$ and $l_1, ...$ are indices of fields that need to be decrypted using MPC and standard encryption technique correspondingly.}
% \label{setup}
% \end{figure*}




% \begin{table*}[]
% \caption{Security Analysis of the pushing model. \text{Differences with the pulling model are highlighted in italics.}}
% \label{push_analysis}
% \begin{tabular}{|p{5cm}|p{8cm}|p{4cm}|}
% \hline
% \textbf{Information} & \textbf{Consequence / Implications} & \textbf{Potential Solution} \\ \hline
% \multirow{2}{*}{\textbf{1. Rule ID and User ID}} & Attacker can link the current execution with previous executions of the same RuleID &  \\ \cline{2-3} 
%  & Attacker can link with executions of other rules installed by the same user / from the same client &  \\ \hline
% \multicolumn{3}{|p{17cm}|}{\textbf{2. Network messages received from trigger service}} \\ \hline
% a.       Presence & \textit{The trigger event has happened} &  Send cover traffic  \\ \hline
% b.       Encrypted trigger data (MPC + AES) & - &  \\ \hline
% c.       Size  & Some fields of the trigger data are missing, and parts of the circuit won’t be executed & Make API always retrun fixed-sized data / Pad message to fixed length \\ \hline
% d.       Time & \textit{The trigger event happens at some frequency} & Send cover traffic \\ \hline
% \multicolumn{3}{|p{17cm}|}{\textbf{3. Network messages sent to action service}} \\ \hline
% a.       Presence & N/A (it should always be present) &  \\ \hline
% b.       Encrypted action data (MPC + AES) & - &  \\ \hline
% c.       Size & N/A (it is determined by 2c trigger data size) &  \\ \hline
% d.       Time & N/A (the time it takes to send action data depends on the execution time of the circuit, which in turns should only depend on the circuit size) &  \\ \hline
% \multicolumn{3}{|p{17cm}|}{\textbf{4. Rule function}} \\ \hline
% \multirow{2}{*}{a.       MPC circuits / function semantics} & Attacker can link with executions of other rules using the same circuit/function &  \\ \cline{2-3} 
%  & If the function has no predicate, then attacker knows the action will be performed if trigger happens & Construct a dummy predicate \\ \hline
% b.       MPC table & - &  \\ \hline
% \multicolumn{3}{|p{17cm}|}{\textbf{5. Semantics of trigger and action services}}  \\ \hline
% a.       URL of the API & Domain knowledge of trigger and action services &  \\ \hline
% b.       OAuth tokens & Attacker can link with executions of other rules using the same  tokens (from the same user) &  \\ \hline
% \end{tabular}
% \end{table*}




==> design_new.tex <==
\section{Design of~\stap}
\label{sec:design}
%One of the goals while designing \stap was to ensure that TAP should continue to
%provide the level abstraction between TS and AS as it provides now. To make TAP
%oblivious of the trigger data $\dt$, we can encrypt the data with a key that is
%only available to the AS. Some types of trigger data, such as an images or media
%files, are never modified by (current) TAPs. For such data, simple encryption
%would suffice to provide confidentiality.  However, for other types of trigger
%data such as numbers of strings, using encryption would prevent computing any
%functions over it.

%We, therefore, use a combination of cryptographic schemes to enable secrecy of
%the trigger data.  % To do so,
% we have to redesign trigger-action platform from ground up. In this section we
% will detail the design of our \stap.
%We first describe the cryptographic schemes used in \stap, and then discuss design details.

% high level overview of our approach: we split trust and do GC

We provide a high-level overview of \name's design, and a detailed discussion of the protocols and the associated design choices. We also discuss how we support string operations, a widely-used class of computations in TAPs, using a novel encoding of deterministic finite automata into garbled circuits. We prove all security claims in Section~\ref{sec:sec_analysis}.


\begin{figure}[t!]
\centerline{\includegraphics[width=0.5\textwidth]{images/TriggerActionSystem.pdf}}
\caption{Overview of \stap.}
\label{fig:arch_overview}
\end{figure}

\subsection{High-level design of \name} 

\figref{fig:arch_overview} shows the structure of \name.  Like a typical trigger-action system, \name has four components: trusted client's device ($\TC$),
\as{TC not always present in a typical TAP though}
trigger service ($\TS$), action service ($\AS$), and a trigger-action platform ($\TAP$). Our design modifies these four components while maintaining the trigger-compute-action paradigm.

\noindent\textbf{Decentralized Trust Model.} In current trigger-action system design, users place all trust within a centralized cloud-based TAP. As we have discussed, this design leaves open a long-term large-scale security and privacy risk. \name borrows a design element from DTAP~\cite{fernandes2018decentralized} and designates the user's client device (smartphone) as the root of trust. Each user \textit{only} trusts their own smartphone, and uses it to program trigger-compute-action rules. As the \name protocols are open-source, we envision a community of developers building client apps, much like we have apps for open protocols like SFTP, Telnet, etc. Thus, the \name cloud component and client app are written by different entities that do not trust each other. \name bootstraps its guarantees on top of this trust model.

%A major difference between our work and
%existing TAPs concerns the role of the client. Recall that the client is a
%smartphone app that users program rules with. In the current TAP design,
%the client and the TAP itself is written by the same entity (e.g., IFTTT or
%Zapier). Similar to prior work~\cite{fernandes2018decentralized},  we require the client to be maintained by an entity
%\textit{other} than the TAP provider. We envision a community of developers
%building clients for our open \stap protocol. The app is possibly also
%open-sourced and vetted for security by the community. With this added trust, we design \name by reusing the architecture of the existing trigger-action systems, 
%but adds some extra functionalities to each component.  As before, $\stap$ has four
%components: trusted client's device ($\TC$), trigger service ($\TS$), action service
%($\AS$), and a trigger-action platform ($\TAP$).  We present a  high-level view of its design in~\figref{fig:arch_overview}. For simplicity, we omit the transmission of data that is already present in current trigger-action system, such as OAuth tokens and user id.

% and
% then hosting them on various marketplaces (e.g., Android or Apple Store). 
% The
% app market model naturally results in a few well-built apps emerging to the
% top. For example, the Google Play store has hundreds of SSH client apps, with
% only a few being highly rated and downloaded. We see a similar situation with
% other open protocols such as Telnet, FTP, etc. Additionally, the open source
% community can independently vet open clients for security issues. Therefore, we
% envision a similar situation for the client in our setting.

\noindent\textbf{Rule Setup.} Using the trusted smartphone app \TC, the user configures a trigger-compute-action rule by choosing the trigger service \TS, the functions to compute over trigger data and the action. This step is the same as current systems. During this process, \TC generates a set of symmetric keys  $\sects$ and $\secas$ that it shares with \TS and \AS respectively (over a TLS connection). Next, the \TC generates a garbled circuit corresponding to the computation over trigger data, and the associated encoding/decoding blobs using a customized protocol (details in next section). 

Two parties derive the encoding blob during setup using $\sects$--- \TC and \TS.\footnote{We choose to transmit $\sects$ to \TS during setup instead of the entire encoding blob for communication efficiency.} The encoding blob allows \TC to encode the user-supplied private constant data into garbled input labels.  



The \TC sends the garbled circuit, encoded constants and encrypted decoding blob to the untrusted \TAP. The decoding blob allows \AS to decode the encoded action data and to decrypt the payload that the TAP does not compute on. We choose to transmit the decoding blob to the \AS for efficiency reasons, and thus, to ensure that the TAP does not modify this blob, \TC encrypts it using $\secas$. 

Note that in our setting, the generator of the garbled circuit is the smartphone client---a trusted entity. This is a key insight and design element that is possible due to the nature of our setting. This allows \name to use efficient semi-honest implementations of garbled circuits and achieve security in the presence of a malicious \TAP. 

The \TC is not needed during rule execution because it has transmitted all information to the other components. This achieves our design principle of keeping the client device offline during rule execution.

%{The installation of a new rule starts with the \textit{rule setup phase} where the user first sets up the necessary rule specifications, such as choosing trigger and action and specifying function details, via its trusted device \TC, similarly to current trigger-action system's model. Additionally in \stap, \TC generates a pair of keys, $\sects$ and $\secas$ which are shared with \TS and \AS, respectively. 
%Next, \TC generates the requisite garbled circuit, and the associated encoding/decoding blobs through a customized protocol. The encoding blob is in fact computed from $\sects$ and allows \TC to encode the user-supplied private constants into garbled input labels. The decoding blob allows \AS to decode garbled action data and decrypt payload, and is encrypted to ensure \AS can only access it when the action needs to be performed and \TAP can never access it.
%Following this, \TC sends the garbled circuit, the garbled constants and the encrypted decoding blob to \TAP. } 

\noindent\textbf{Rule Execution.}  When new trigger data is available, the \TS will encode the data (using the encoding blob it already derived during setup) and encrypt any payload data. It then transmits the ciphertext to the \TAP that will run the garbled circuit. The \TAP finally transmits the output of evaluation (garbled action data) and the encrypted decoding blob to the \AS that can decode to the plaintext result using $\secas$. The \TS and \AS only perform simple encoding and decoding of labels---fixed functionality independent of the trigger-action rule semantics, thus maintaining their RESTful nature. We believe that \TS and \AS are well-motivated to support these additional operations, in exchanged for enhanced security. Indeed, current end-point services are concerned about privacy of user data. For example, GMail recently removed their IFTTT triggers citing privacy concerns~\cite{gmail-ifttt-removal}. 

 In our setting, the full evaluation of the garbled circuit is split between the untrusted \TAP that executes the circuit to produce encoded output labels and the semi-honest \AS that decodes these result from the labels. This, in combination with the trusted generator (smartphone) allows \name to efficiently achieve the execution authenticity property of GCs using a hashing scheme (Section~\ref{sec:design-rationale}), even when \TAP itself is malicious. 

%First, \TS computes the encoding blob from $\sects$, and uses it to encode its private trigger data and to encrypt payload, which are then sent to \TAP. \TAP  evaluates the garbled circuit on the garbled trigger data and the garbled user-supplied constants to compute the garbled action data.In the final step, \AS decrypts the decoding blob using $\secas$ and learns the plaintext data/payload. 

\noindent\textbf{Reset Phase.}
After each rule execution phase, \name discards the used garbled circuit. Thus, the client has to periodically generate a set of garbled circuits with associated information and transmit those to \TAP. This happens \emph{asynchronously} from rule execution. For example, the client can generate and transmit a batch of circuits at night while the phone is being charged.  Thus, the client does \emph{not} need to be online during rule execution. Our evaluation demonstrates that \ef{put claim.}


%In particular, with \name's design we solve the following challenges efficiently:
%\begin{newitemize}
%\item offline behavior of \TC during rule execution;
%\item protection against a malicious \TAP while still using a semi-honest model based implementation;
%\item ensuring that \AS learns about the action data and payload only when action needs to be performed (i.e., $f_1(x,c_1)=\true)$;
%\end{newitemize}
%These are covered in detail in Section \ref{sec:design-rationale}.
% \name achieves security (we formally prove guarantees in
% Section~\ref{sec:security-analysis}) in the presence of a malicious circuit
% evaluator (i.e., TAP) that can arbitrarily deviate from the rule execution
% protocol. %because of our decentralized design that splits trust --- every user has
% their own trusted client that generates garbled circuits.



% To meet our security requirements specified in the threat model, we would use
% a garbling scheme that have these two security properties.



% \rcnote{Can we just borrow from emp-toolkit that their scheme provides
%   obliviousness and authenticity? and only prove the small delta that we have.}

% We present every operations in Boolean circuit for garbling. This is
% straightforward for arithmetic operations, however, not so for string
% operations. Most of the string operations can be captured using a subset of
% regular expressions. We therefore created a simple engine to convert regular
% expression-based operations into Boolean circuit. The details of our operation
% is given in~\appref{app:bool-regex}.

% From our analysis of rules in~\secref{sec:rules}, we found that arithmetic
% functions are not used in conjunction with arithmetic operations. While in
% theory, garbled circuit can be use to solve such mixed-operations, we found that
% our garbling scheme will become computationally and bandwidth-wise
% expensive. Therefore, currently, we don't support using both arithmetic and
% string operations in the same function. We leave for future studies to explore
% efficient ways to use the two operations in one function, if
% required. \rcnote{the language is quite loose.}

% \ef{discuss abstract model and how we derived it including the set of supported functions, then discuss concrete design, and finally show security arguments}

% % abstract model
% % concrete design:
% %  -- system-level design
% %  -- protocol design for numerics, string DFA
% % security arguments

\subsection{Architecture}\label{sec:arch}
% \ef{this should flow as: system architecture diagram plus explanation of each component, discuss an example rule and how it would execute. When we introcude the Trusted Client, we should motivate why this design choice is reasonable.}
% \figref{fig:arch} shows the architecture of \name.

We now describe \name's customized protocol that uses a symmetric-key encryption scheme and garbled circuits.
  
%\begin{comment}
%In this section, we first start with key differences between a typical 2-party secure function evaluation using garbled circuits (discussed in Section \ref{sec:crypto_tap}) and our setting.\begin{itemize}
%\item First, there are four parties in our setting - client's device ($\TC$), trigger service ($\TS$), action service
%($\AS$), and a trigger-action platform ($\TAP$). As discussed in the preceding subsection, \TC and  \TS jointly act as the \textit{generator} while  \TAP and  \AS emulate the roles of the \textit{evaluator}.
%\item Second, the "evaluators" in our setting,  \TAP and  \AS, do  not have any private input. The function is computed only on the input from  \TC ($\cone$ and $\ctwo$) and  \TS ($x$).  
%\item Third, the trust assumptions of the two constituting parties of both the generators and the evaluators are incompatible. Specifically in %the case of the generators, 
%while  \TC is completely trusted,  \TS is assumed to behave semi-honestly. For the evaluators, we assume  \AS to be semi-honest while  \TAP can %act maliciously.
%\end{itemize}
%  In the following paragraphs, we describe how \name to customize the generic 2-party garbled circuit protocol in the trigger-action platform to account for the aforementioned changes.  
  %%\\\\\\\\\\\\\\\\\\\\\\\\\\\\\\

%In \name, $\TC$ participates during the rule setup phase, and then periodically
%generates and sends garbled circuits to $\TAP$. The trigger and action
%services apply a shim over their API endpoints that transparently translates
%between the encoded and decoded versions of their data. Instead of computing the
%function over plaintext trigger data, $\TAP$ will evaluate the garbled circuit
%over the encoded trigger data.
%\end{comment}

\paragraph{Rule Setup (performed on the trusted client).}
As discussed, the user creates a trigger-compute-action rule with the help of the trusted client app. This involves specifying the predicate $\fone$, the data transformation $\ftwo$, and any user-supplied constants ($\cone$ and $\ctwo$) using a click-through interface. Similar to current systems, the \TC negotiates OAuth tokens corresponding to the trigger and action service. Unique to our work, the \TC generates a rule ID $j$ initialized to zero, and two secret keys $\sects, \secas \in \zo^\keylen$. \name uses the rule ID

As with current systems, the \TC negotiates OAuth tokens corresponding to the rule, and then distributes those tokens, and a description of the rule to the \TAP. 


{The rule setup phase happens every time a new rule is installed in \name. In this phase, the user connects a trigger
service $\TS$ with an action service $\AS$ by acquiring the necessary OAuth tokens
from $\TS$ and $\AS$. This is similar to its functionality in current trigger-action platforms. Additionally, in the push model of trigger-action systems, $\TAP$ generates a secret callback address for $\TS$ so that $\TS$ can actively
transmit trigger data. The user also specifies the functions
($\fone$ and $\ftwo$) to be evaluated at $\TAP$ via a click-through user
interface and, if required, the constant parameters ($\cone$ and $\ctwo$).
Every rule is assigned a rule id. 
\name additionally requires \TC to generate two secret keys $\sects, \secas \in \zo^\keylen$ and to initialize a circuit id $j$ to $0$. Recall that a circuit is discarded after a single use; the circuit id $j$ hence helps in keeping track of the circuit to use in the current iteration of rule execution.}
% Next, \name additionally requires \TC to generate and store two random strings $\sects, \secas \in \zo^\keylen$, which are secret keys to be shared with \TS and \AS, respectively, and a random integer $j$, which is used as the circuit id. $\sects$ and $j$ are sent to \TS while $\secas$ and $j$ are sent to \AS during this setup phase.
% \rcnote{Why do you have to generate/send the circuit id $j$ during setup? Do you mean rule-id? I commented it out; if necessary you can uncomment it back. }
% \yc{$j$ here refers to the initial circuit id, which will get incremented after each rule execution}

The rule id, callback addresses, the OAuth tokens are uploaded to $\TS$, $\AS$,
and $\TAP$ accordingly as they are done in current trigger-action systems. However,
the user-supplied constants are stored locally on~$\TC$. The tuple $(j,\sects)$ is shared with $\TS$, and while $(j,\secas)$ is shared with $\AS$. 


% \begin{figure}[t]
% \centerline{\includegraphics[width=0.4\textwidth]{images/rule_setup_execution_11.png}}
% \caption{Diagram showing the high-level architecture of \stap. The client $\TC$ garbles the circuits and forwards them to \TS,\TAP, and \AS. During rule execution we don't need the client to be online.}
% \label{fig:arch}
% \end{figure}
\def\jprev{j_{\textsf{\tiny prev}}}
\begin{figure}[t]
  \gamesfontsize
  \hspace{-2em}
  \hfpagess{0.23}{0.24}{
    \underline{\textsf{CktGarbling}$\left((f, \const), (j, \sects, \secas)\right)$}:\\[2pt]
    $\eis \gets \H(\sects \concat j \| 0) $\\
    $\eir \gets \H(\sects \concat j \concat 1) \lor 0^{\keylen-1}1 $\\
    $\key \gets \H(\sects \concat j \concat 2) $\\
    % $\ei\gets(\eis,\eir)$\\
    % $(F, \di', h) \gets \Gb'\left((\eis,\eir), f\right)$\\
    $(F, \wlabel^{w_0}_0, \ldots, \wlabel^{w_m}_0) \gets \Gb'(f, \ei)$\\
    $d' \gets (\textsf{lsb}(\wlabel^{w_1}_0), \ldots, \textsf{lsb}(\wlabel^{w_m}_0))$\\
    $h \gets \H(\wlabel^{w_1}_0 \concat \ldots \concat \wlabel^{w_m}_0)$\\
    $\encd \getsr \skeenc(L^{w_0}_1 \oplus \secas, (j, k, \eir, d', h)) $\\
    $C \gets \En(\ei, \const)$\\
    % $j \gets j + 1$\\
    Return $j, F, C, \encd$\\[2pt]

    \underline{\textsf{TriggerExec}$\left((\dt, \payload), (\sects, j)\right)$:}\\[2pt]
    $\eis \gets \H(\sects \concat j \concat 0)$\\
    $\eir \gets \H(\sects \concat j \concat 1) \lor 0^{\keylen-1}1  $\\
    $\key \gets \H(\sects \concat j \concat 2) $\\
    % $\ei\gets(\eis,\eir)$\\
    $\LT \gets \En\left((\eis,\eir), \dt\right)$\\
    $t \gets \textsf{CurrentTime()} $\\
    $ct \getsr \skeenc(k, (t, \payload))$\\
    $\return j, \LT, ct$
   }
  {
    \underline{\textsf{PlatformExec}$\left((j,X,ct), (F,C,\encd)\right)$:}\\[2pt]
    $Y \gets \Ev(F, (\LT, C))$\\
    $\return j, \LA, ct,\encd$\\[2pt]
    
    \underline{\textsf{ActionExec}$\left((j, \LA, ct,\encd), \,\secas, \jprev\right)$:}\\[2pt]\\
    Parse $\LA$ as $(\wlabel^{w_0}, \wlabel^{w_1}, \ldots, \wlabel^{w_m})$\\
    $z\gets \skedec(\wlabel^{w_0} \oplus \secas, \encd)$\\
    If $z = \bot$ then \ $\return \bot$\\
    $(j'', k, \eir, d', h) \gets z$\\
    %if $(j''==0)$ then $j_{prev} \gets 0$
    $y \gets \De\left(d', \LA\right)$\\
    $g\gets \bot$\\
    For $i\gets 1$ to $m$ do\\
    \mytab If $y_i = \false\;$ then $\;g\gets g\concat\wlabel^{w_i}$ \\
    \mytab Else $\;g\gets g \concat (\wlabel^{w_i}\oplus\eir)$\\
    % $h' \gets \H\left( (\wlabel^{w_1} \oplus y_1 \eir) \| \ldots \| (\wlabel^{w_m} \oplus y_m \eir) \right)$\\
    $h'' \gets \H(g)$\\
    $(t, \payload) \gets \skedec(k, ct)$\\
    $t''\gets \textsf{CurrentTime}()$\\
    If $t''> t+\delay$ or $h \ne h''$ or $j \ne j''$\\
    \hspace{.1em} or $j''\ne \jprev+1$ then\\
    $\mytab\return~\bot$\\
    Set $\jprev = j$\\
    $\return y, \payload$
  }
  
  \caption{Circuit generation and rule execution protocols for $\stap$.
    $\wlabel^{w_0}_1$ denotes the $\true$ label chosen of the first output wire $w_0$;
    $\delay$ is a threshold parameter used to ensure the freshness of a
    trigger; $\jprev$ is the last seen circuit id, initialized during rule setup by
    \TC. The \textsf{CircuitGarbling} is run by the client $\TC$
    asynchronously of the actual rule execution.  The remaining three functions
    are run by \TS, \TAP, and \AS during rule execution.
}
  \label{fig:algo}
\end{figure}



\paragraph{Circuit garbling (performed on the trusted client).} 
{After setting up the rule specifications, \TC generates the garbled circuit for the function to be computed and its associated encoding/decoding information. 
Without loss of generality, we assume 
$\fone\Colon\zo^n\times\zo^n\to\zo$ and
$\ftwo\Colon\zo^n\times\zo^n\to\zo^m$. For notational simplicity, we denote  $f\Colon\zo^n\times\zo^{2n}\to\zo^{m+1}$, such that
$f(\dt, \const) = \fone(x, \cone)\|\ftwo(x, \ctwo), \const=(\cone, \ctwo) \in\zo^{2n}$. Additionally, let $\H: \zo^*\to\zo^{\kappa}$ denote a cryptographic hash function.}
%We only mention $\fone$ and $\ftwo$ or $\cone$ and $\ctwo$ when required.


\paragraph{\textnormal{\emph{Encoding Blob.}}}{ \TC first generates the encoding information for the garbling scheme's encoding function (\En) as follows. It generates two bitstrings $(\eis, \eir) \in \zo^{2\keylen}, $ using the hash of $\sects \concat j$. Recall, that a garbled circuit associates each wire $w$ with two random labels $\wlabel_1^w$ and $\wlabel^w_0$ --- representing the $\true$ and $\false$
values. $\eis$ is the random seed used for generating the $\false$ labels of the input wires (as described below) while $\eir$ is a global offset used for the standard free XOR optimization~\cite{kolesnikov2008improved}. Thus
$\ei=(\eis, \eir)$ constitutes the encoding information. 
Additionally, \TC generates a key $\key \in \zo^\keylen$, which is used to
encrypt trigger payload data~$\payload$. We refer to $(\ei, \key)$ as the encoding blob.}

\paragraph{\textnormal{\emph{Garbled Circuit.}}}To generate the garbled circuit $F$ for function $f$, first the labels 
for every input wire $w$ are computed as $\wlabel^w_0 = \H(\eis, w)$ and
$\wlabel^w_1 = \wlabel^w_0\oplus \eir$ (assuming  wire index $w$ is represented as a fixed-length bitstring).  The rest of the computation (generation of labels for the non-input wires) can proceed as per standard techniques including row-reduction \cite{NPS99}, half-gate \cite{zahur2015two} and point-and-permute optimizations \cite{BMR90,MNP+04}. 

% We refer the reader
% to~\cite{zahur2015two} for details on the garbling function.

% Note that, \name's customization only affects the encoding of the input wires (corresponding to $x$ and $(c_1,c_2)$). Hence, in addition to the free XOR \cite{kolesnikov2008improved} and point and permute optimizations \cite{BMR90},\cite{MNP+04}, the aforementioned garbled circuit protocol supports the standard row-reduction \cite{NPS99} and half-gate \cite{zahur2015two} optimizations as well. 

% We use $\Gb'$ to denote the non-standard garbling function that takes a function $f$ (represented as a
% Boolean circuit) and required encoding information $e$ and returns a garbled
% version of $f$ along with the $\false$ labels of all output wires.  
% 


\newcommand{\hwlabel}{h}
\paragraph{\textnormal{\emph{Encrypted Decoding Blob.}}}  {The decoding blob consists of information necessary for \AS to decode the labels of output wires (which corresponds to the action data $y$) and decrypt the payload. Let the output wires be
$(w_0, w_1, \ldots, w_m)$, where $w_0$ corresponds to the output wire of $\fone$, and
the remaining $m$ wires correspond to those of $\ftwo$. Recall that the decoding information $d$ of standard garbled circuits enables decoding output labels back to the corresponding plaintext bits. Following standard practices \cite{zahur2015two}, $d$ typically contains the least significant bits of the $\false$ label of each output wire ($\textsf{lsb}(\wlabel^{w_0}_0), \ldots, \textsf{lsb}(\wlabel^{w_m}_0)$). In \name, \TC modifies this decoding information slightly and computes the decoding blob as follows. First, the first bit $\textsf{lsb}(\wlabel^{w_0}_0)$ is dropped from $d$. We refer to this shorter decoding table as $d'$. Second, the hash of all the $\false$ labels of $\ftwo$'s output wires is computed, $h \gets \H(\wlabel^{w_1}_0 \concat \ldots \concat \wlabel^{w_m}_0)$ and added to the decoding blob. Third, the payload key $k$, the XOR offset $\eir$, and the current circuit id $j$ are included in the decoding blob as well. Finally,  the entire decoding blob is encrypted under a symmetric-key encryption scheme with two keys: $\secas$, the secret key shared with \AS, and $\wlabel_1^{w_0}$, the $\true$ label of $\fone$'s output wire $w_0$, to obtain $\encd \getsr \skeenc(L^{w_0}_1 \oplus \secas, (j, k, \eir, d', h))$. We explain the rationale behind these changes later in Section \ref{sec:design-rationale}}. %This encryption ensures that \TAP will never learn the decoding blob (since it does not have $\secas$) while \ASwill only be able to learn the decoding blob when the predicate $\fone$ is evaluated true (otherwise it will receive $\wlabel_0^{w_0}$ instead of $\wlabel_1^{w_0}$). We denote this encrypted decoding blob as $\encd$.

\paragraph{\textnormal{\emph{Encoding User Constants.}}} {\TC computes the labels for the user-provided constants $c$ as $C \gets \En(\ei,\const)$ using the encoding information $\ei$. }

{\TC sends $(j, F, C,\encd)$ to the \TAP. Before garbling the next circuit, \TC increments the circuit id $j$ by 1.  We refer to \name's modified garbling scheme as $\Gb'$ and the entire protocol for garbling circuits as discussed above is presented algorithmically in the function \textsf{CktGarbling} in Fig. \ref{fig:algo}.}
  

% When \AS
% receives a tuple of labels $(\wlabel^{w_1},\ldots,\wlabel^{w_m})$ from the \TAP after circuit evaluation, it computes $\wlabel^{w_i}_0 = \wlabel^{w_i}_{y_i} \oplus y_i \eir$ for each output wire after getting $y_i$ from the decoding procedure and the hash of
% their concatenation. If the new hash does
% not equal to the one received from \TC, the decoding procedure will fail, which allows us to
% catch if a malicious TAP lying about the output of the function $f$.


%the value of the output wire $w_i$ is set to $b$ if
%$\exists\ b\in\zo,\,\H(\wlabel^{w_i}) = \H(\wlabel^{w_i}_b)$, and $\bot$,
%otherwise.  



%Also, the
%$hashing protects the global XOR-offset $\eir$ from the action service.  



% Finally, we don't want \name to learn about the decoding information, nor should the action service  when
% output of $\fone$ is $\false$. % is the first wire $w_0$ is set to zero.
% We, therefore, encrypt the decoding information $d$ with the $\true$ label of
% the output wire $w_0$ (i.e., $\wlabel_1^{w_0}$) and \AS's secret string: the client computes
% $\encd\getsr\skeenc(\wlabel^{w_0}_1 \oplus \secas, (d, k, h, \eir, j))$. The encryption ensures 
% \name will never learn any results of its output
% while \AS
% will only be able to learn the result of $\ftwo$ when the predicate $\fone$ is
% true.

%would not learn anything about the decoding information without receiving the
%correct $\true$ label $\wlabel_1^{w_0}$ from \TAP. 

% Note
% However, the way
% labels are generated, we cannot send $\{L^w_0, L^w_1\}$ for each output wire
% $w$; else the trigger service will learn the XOR-offset $R = L^w_0\oplus L^w_1$,
% which enables inquisitive $\TS$ to learn about the decoding information $d$,
% even when the the first bit of the output of $f$ (or $\fone$ evaluates to
% $\false$).



% First, the client generates four
% random strings, $\ei_\dt, \ei_c, R, k \in \{0,1\}^\keylen$:
% \begin{itemize}
% 	\item $\ei_\dt$ and $\ei_c$ are the seeds of the PRG: $\{ 0, 1 \}^\keylen \to \{ 0, 1 \}^l $, where $l \gg \keylen$.
% 	\item $R$ is the free-XOR offset common to all wires. To enable the point-and-permute technique, the least significant (last) bit of $R$ is manually set to 1.
% 	\item $k$ is the key to the symmetric-key encryption scheme.
% \end{itemize}

% Then for each input wire that belongs to the trigger data $\dt$, we use $\PRG(\ei_\dt)$ to generate its FALSE label, i.e. the $i$-th input wire will use the $ik$-th to $i(k+1)$-th bits from the output of PRG as its FALSE label. The TRUE label is computed by xor-ing the FALSE label with $R$. \yc{Describe this in mathematical terms?} Similarly, the labels for the input wires that belongs to $\cone$ or $\ctwo$ are generated using $\PRG(\ei_c)$.

% Next, the garbling protocol $\Gb(1^\keylen, (\fone, \ftwo))$ is executed, which will produce
% \begin{itemize}
% 	\item The TRUE and FALSE labels for each wire in the circuit,
% 	\item $\Fone$ and $\Ftwo$, the garbled version of $\fone$ and $\ftwo$.
% \end{itemize}

% Finally, \TC creates a unique identifier $j$ for this execution and sends
% \begin{itemize}
% 	\item $j, e^{(j)}$ to \TS, where $e^{(j)} \gets (\ei_\dt, R, k)$;
% 	\item $j, F^{(j)}, C^{(j)}$ to \TAP, where $F^{(j)} \gets (\Fone, \Ftwo)$ and $C^{(j)} \gets (C_1, C_2)$, which are the labels corresponding to $\cone, \ctwo$;
% 	\item $j, d^{(j)}$ to \AS, where
% 	\begin{itemize}
% 	    \item $d^{(j)} \gets (d_{f_1}, \Enc_{L_1^p}(d_{f_2}, k)) $,
% 		\item $d_{f_1} = \textsf{lsb}(L_0^p)$ is the least significant bit of the FALSE label for $f_1$'s output wire,
% 		\item $d_{f_2}$ contains the hashes (computed via hash function $H$) of the TRUE and FALSE labels for every $f_2$'s output wire,
% 		\item $L_1^p$ is the TRUE label for $f_1$'s output wire.
% 	\end{itemize}
 
% \end{itemize}
% \yc{check notation consistency}


% We extend this functionality of the trusted client to periodically generate the
% garbled circuits and associated encoding and decoding information and distribute
% them to the TS, TAP, and AS. We believe this periodic engagement is practical,
% and as we show via our experiments, computationally feasible for average
% cellphones or computers.  \rcnote{Check with DTAP paper to find more plausible
%   argument of the trusted client.}

\paragraph{Rule execution (does not involve client).}
{In this section, we describe \name's workflow for executing a rule in the event of the corresponding trigger. %When a trigger event happens, \TS sends the event data to the callback URL provided by \TAP. \TAP evaluates the function $f$ in an oblivious manner and forwards the output to the action service. 
Again we omit the standard OAuth authorization steps (refer to \cite{fernandes2018decentralized} for details).}

{First, $\TS$ uses $\sects$ and the circuit id $j$ to generate the encoding blob in the same way as \TC. Next, it encodes the trigger data $\dt$ (its input to function $f)$ using the garbling scheme's encoding function as the garbled input $X\gets \En(\ei,\dt)$ and encrypts the payload 
$\payload$ under a symmetric-key encryption scheme with the key $\key$ to compute $ct\getsr\skeenc(k, (t, \payload))$ where $\ts$ is the current timestamp. Finally, \TS forwards the message $(j, X, ct)$ to
TAP and increments $j$ by 1. \TS's operations in the rule execution phase is represented by the function \textsf{TriggerExec} in Fig.~\ref{fig:algo}.}

{\TAP, on receiving a trigger message $(j, X, ct)$, retrieves the corresponding garbled circuit $F$, garbled constants $C$, and the encrypted decoding blob $\encd$ using the circuit id $j$. Next, \TAP evaluates $F$ to obtain the garbled action data $Y\gets \Ev(F,(X,C))$ and forwards the tuple $(j, Y, ct, \encd)$ to the \AS. Function \textsf{PlatformExec} in Fig. \ref{fig:algo} presents the action of \TAP in this phase. }

{After receiving a message from \TAP, %\AS first verifies that the received circuit id $j$ is one more than $j'$, the last seen circuit id. %greater than all the other idsseen previously. 
 \AS decrypt $\encd$ to obtain the decoding blob, which will succeed only when $\fone$ evaluates to $\true$ (i.e.  $\wlabel^{w_0} = \wlabel_1^{w_0}$). In the event \AS obtains the decoding blob, it uses $(d', \key)$ to obtain the final output $(\ftwo(x,\ctwo), \payload)$ in plaintext.  However, \AS would also terminate if the message
from \TAP is malformed (i.e.\ hash of labels is inconsistent or decryption fails) or stale (i.e.\ trigger timestamp is old) or the circuit ids are inconsistent. The operations of \AS discussed above is presented in the function \textsf{ActionExec} in Fig. \ref{fig:algo}.} %The authenticity of the message is determined by converting each received label (except the first one) to the corresponding $\false$ label and then comparing the new hash with the hash embedded in the decoding blob, while the staleness is checked through the timestamp $t$ and circuit id $j$. 
%The final output of \textsf{ActionExec}, other than $\bot$, is fed to the action API.

%Note that for every rule, \TC periodically and asynchronously generates a set of garbled circuits and the associated keys $(\sects,\sects)$. 




\subsection{Need for customization of GCs in \name}\label{sec:design-rationale}

{Now, let us revisit \name's workflow and understand the need for the customized garbled cicruit protocol. First, we start with the key differences in behavior between a typical 2-party secure function evaluation using garbled circuits (discussed in Section \ref{sec:crypto_tap}) and our setting.
\begin{itemize}
\item First, there are four parties in our setting. As discussed in the preceding paragraphs, \TC generates the garbled circuit via $\Gb'$ and then, both \TC and \TS use $\En(e,\cdot)$ to directly encode their respective inputs. Thus, \TC and \TS jointly act as the \textit{generator}. On the other hand, \TAP evaluates the garbled circuit via $\Ev(F,\cdot)$ while  \AS decodes the final plaintext output via $\De(d',\cdot)$. Thus, both \TAP and \AS jointly emulate the role of the \textit{evaluator} in our setting.
\item Second, the ``evaluators'' in our setting, \TAP and \AS, do  not have any private input. The function is computed only on the input from the \TC ($\cone$ and $\ctwo$) and the \TS ($x$). Hence, \name does not require the oblivious transfer protocol.  
\item Third, the trust assumptions of the two constituting parties of both the generators and the evaluators are incompatible. Specifically in the case of the generators, 
while \TC is completely trusted, \TS is assumed to behave semi-honestly. For the evaluators, we assume  \AS to be semi-honest but \TAP can act maliciously.
\end{itemize}
Next, we highlight the computations where \name differs from generic 2-party implementation of GCs and explain the rationale behind these choices in the light of our design goals (Section \ref{sec:design-goals}) and the characteristics of our setting.
Specifically, \name's customized protocol differs in the following ways:
 \begin{itemize}
     \item \textit{Generation of the encoding information}: In \name, the encoding information is computed from the key $\sects$ instead of being generated by the garbling scheme $\Gb'$. This is necessary to ensure that \TS is able to encode its input ($\dt$) efficiently during rule execution without any additional communication with \TC.  This achieves our design goal of ensuring that the users are offline during rule executions.  However, this change does not violate the input privacy guarantees of the garbled circuit as proved by Thms. \ref{thm:TAP1},\ref{thm:AS} and \ref{thm:TS}. Additionally, in the event of a trigger, \TS is required to only encode its trigger data irrespective of the function to be computed. This is in tandem with our design goal of a RESTful \TS.
     \item \textit{Decoding of the first output wire}: Recall, that $\textsf{lsb}(\wlabel^{w_0}_0)$ is dropped from the decoding information $d'$. Instead, the first output wire $w_0$ (i.e, the output of $\fone$) is decoded via an encryption layer. Specifically, recall that the decoding blob (which contains the decoding information $d'$ and payload key $\key$) is encrypted under two keys: $\secas$ and $\wlabel_1^{w_0}$. Hence, the decryption is successful and \AS learns the decoding blob only when it receives $\wlabel_1^{w_0}$, the $\true$ label of $w_0$. This meets our privacy requirement that \AS should not learn about $\ftwo(x,\ctwo)$ or $\dtp$ when $\fone(x,\cone)=\false$. This is formally proved by Thm. \ref{thm:AS}. Note that the encryption under $\secas$ protects the decoding blob from the \TAP (Thm. \ref{thm:TAP1}).
     \item \textit{Ensuring authenticity of output labels}: The decoding blob requires two additional information $h=\H(\wlabel^{w_1}_0 \concat \ldots \concat \wlabel^{w_m}_0)$ and the XOR offset $\eir$. This is to ensure the authenticity of the output labels $Y$ received from the malicious \TAP.
     Standard techniques to ensure such authenticity require the hashes of both $\true$ and $\false$ labels for every output wire \cite{zahur2015two}. However, since \AS does not have access to the garbled circuit $F$ and the encoded inputs $(X,C)$ in \name, it is safe to disclose $\eir$ to \AS (Thm. \ref{thm:AS}). Thus, \AS can compute $\wlabel^{w_1}_0, \ldots, \wlabel^{w_m}_0$ (see \textsf{ActionExec} in Fig. \ref{fig:algo}) from the output labels and check whether \TAP has returned inauthentic labels. Therefore, only a single hash $h$ is sufficient in our case.
     This is proven formally by Thm. \ref{thm:TAP2}.
    Note that this small modification enables \name to protect against a malicious \TAP while still using a semi-honest model based (hence more efficient) implementation  of garble circuits. The main reason behind this is that our "generators" are assumed to be at least semi-honest (see Section. \ref{sec:sec_analysis} for more details).% This leads to performance efficiency in \name since typically the malicious model based implementations for any cryptographic protocol are significantly costlier than  their semi-honest model based implementations.
 \end{itemize}}




  
% Each service uses $j$ to synchronize the garbled circuits and associated
% information to use. Therefore, if a service does not find a valid database entry
% for a circuit id $j$, the associated message is silently dropped. Also, after a
% circuit id is used, each service is supposed to delete the associated
% information from their database. \TS will never reuse a circuit for encoding
% its trigger data. This provides forward secrecy to the system in case the
% attacker compromises both \TS and \AS.  The client $\TC$ periodically generates a number of circuits and sends them to \TS, \AS, and \TAP. 


\subsection{Converting functions to Boolean circuits}\label{sec:boolfunc}
% \subsection{Converting string operations to garbled circuits} 
% \label{sec:gc-ops-string}
While in theory any computable function can be converted into Boolean circuits,
and therefore can be computed using garbled circuits, in practice
they can be very expensive. For example, most GC libraries support Boolean and
arithmetic operations natively, but none support string operations out of box.
%emulating strings
%operations over array of characters is also difficult.  
We therefore devise a
novel method to convert string operations requiring regular expressions into
Boolean circuits that are efficient for GCs.

\paragraph{Converting DFAs into Garbled Circuits.}  Based on our analysis of the operations used in commercial TAPs  (Section \ref{sec:supported-functions}), we observe that a large fraction of them are string operations that can be expressed as matching and substring extraction/replacement. Regular expressions can be converted into deterministic finite automaton (DFA) for easy evaluation.
Mohassel et al.~\cite{mohassel2012efficient} introduced an oblivious deterministic finite automata (Obliv-DFA) approach to match regular expressions in a secure 2-party computation setting. However, their approach requires a 
custom non-GC based protocol and 
cannot be easily extended to support substring extractions and replacements.

Therefore, we implement a purely circuit-based approach to efficiently match a
DFA with an input string and support substring extractions and replacements, particularly leveraging the fact XOR gates can be computed
for ``free'' in a garbled circuit. By
converting DFA matching to a Boolean circuit, we keep our existing garbled
circuit infrastructure, and retain the same security properties.

We describe the details of how to convert DFAs into Boolean circuits and how to extend to that to perform substring replacement and extraction in~\appref{app:regex}. We assume the input string is of fixed length and \TS unambiguously pads the string if the string is smaller.

For string replacement, we replace the matched substrings with special symbols, and \AS replaces them with the replacement string. The replacement string is encrypted with the hash of the labels for the special symbol, so that \AS can only learn about the replacement string if there exists such a replacement. 
% In \secref{sec:arch}, we refer $\fone$ and $\ftwo$ as Boolean circuits of fixed
% input and output sizes, instead of generic functions. While certain operations
% are quite straight forward to evaluate in garbled circuit (GC), some are
% not. For example, supporting Boolean and arithmetic operations is quite straight
% forward. However, string operations, such as the one involve regular expressions
% (e.g., \texttt{extract\_phone}) is not efficiently handled by standard GCs.


\paragraph{Supported Functions.} 
By incorporating the above techniques, we can use garbled circuit to compute
practically all functions listed in~\figref{fig:functions} with three exceptions
(\texttt{format}, \texttt{strip\_html}, and \texttt{html2markdown}). We sketch
the implementation details for each supported function in~\appref{app:func-impl}. Based on our dataset collected in \secref{sec:supported-functions}, this
set of operations enables \name to support 93.4\% of the function-dependent
rules published on Zapier and all top 500 IFTTT rules.

It is possible to convert the remaining three unsupported functions to Boolean circuit, as well, but the resulting circuit will be very large (for example, we need to build a full-blown parser to find HTML tags). In addition, we argue that these functions are only used for formatting, and do not require any sensitive user input. Therefore, we can choose to run them in \AS or \TS directly on plaintext data and still retain our security goals. 


%Standard garbled circuits efficiently support Boolean and arithmetic operations. Unfortunately, string operations can become inefficient with current frameworks because they will be broken down into very large circuits. Thus, Mohassel et al. introduced an efficient deterministic finite automaton (DFA) approach to support string operations that can be expressed using regular expression (e.g., pattern matching)~\cite{mohassel2010}. However, this approach does not meet our requirements because the party who holds the secret data must evaluate the DFA circuit. In our setting, the \TS holds the secret data. As discussed in Section~\ref{sec:towards}, this puts undue burden on the \TS and breaks the abstraction between \TS, \TAP, and \AS. However, we take inspiration from this approach and build an efficient scheme that converts a DFA into garbled circuits using a custom state encoding scheme. We go beyond regular expressions and also introduce techniques to perform substring extraction and replacement. We discuss our approach to matching regular expressions with garbled circuits next. Appendix~\ref{app:regex-extract} contains a discussion of how we extend this protocol to perform extraction and replacement.

% \subsubsection{Boolean and Numeric} 
% Existing secure multi-party computation frameworks like EMP toolkit~\cite{emp-toolkit} support Boolean and integer or float operations efficiently. We use this support without any modifications.

% \paragraph{Input and output representations.} 
% If a field in the trigger data is a string, we require the \TS to first pad it to 
% a fixed length by appending some predetermined padding characters, as the length of the string may leak the actual content in the string when the input space is small. Then the string is encoded into a fixed-length bitstring $\vecx = (x_1,\ldots,x_n)$ where $x_i\in\zo$ before feed into the encoding function $\En$. Similarly, if an output field is a string, its size should also be fixed to some predetermined length. Therefore, 
% it is the duty of \AS to remove the padding characters after it retrieves the plaintext output.


% \paragraph{Converting DFAs into circuits.}

% We give a description of our approach below. A more concrete explanation on how to support substring extraction and replacement is presented in Appendix \ref{app:bool-regex}.
% Let $\dfa$ be a DFA, defined as a five-tuple,
% $\dfa = (\states, \alphabet, \trans, \State_0, \finalstates)$, where $\states$
% is the set of states, $\alphabet$ is the set of alphabets, $\State_0$ is the
% initial state, and $\finalstates$ is the final state. The transition function
% $\trans$ takes a state and an alphabet and returns the next state; therefore,
% $\trans\Colon\states\times\alphabet\to\states$.  As every string is a
% bitstring, we have $\alphabet=\zo$. Let $\nstates = |\states|$ be total number of states. Without loss of generality, we assume $\states = \mathbb{Z}_q  = \{1, \dots, q\}$.

% Let $\transstring$ be a function that takes a string as input and outputs the
% final state of the DFA after consuming the whole string starting from the state
% $\state_0$, %
% \bnm \transstring(\vecx) = \trans(\ldots\trans(\trans(\state_0,
% x_1),x_2),\ldots, x_n)  \enm If $\transstring(\vecx)\in\finalstates$, then
% $\vecx$ is accepted by the DFA, which means the string matches the regular
% expression.

% We encode each state into a bit-vector of size $\nstates$ using one-hot encoding. 
% We use $\State$ to denote the encoding of a state $\state \in \states$, and $\State^j$ represents the $j$-the bit of $\State$, where $\State_0^s = 1$ and $\State^j = 0$ for any $j \ne s$. 
% Therefore, the output of the DFA becomes 
% \bnm \Transstring(\vecx) = \Trans(\ldots\Trans(\Trans(\State_0,
% x_1),x_2),\ldots, x_n)  \enm
% where $\Trans$ is the transition function that operates on the encoded states.

% We also define two sets for each state $s$, $P_0^\state$ and $P_1^\state$, where 
% \bnm P_b^s = \{i\suchthat\trans(i,b) = j\} \enm for $b\in\zo$.


% %We will now specify the new transition function $\Delta$ is represented as a Boolean circuit. 
% We now discuss how we represent the transition function as a Boolean circuit, suitable for use with any standard frameworks that support free XOR optimizations. Let
% $T = \Trans(S, x)$. We can observe that $T^j=1$ if and only if either $x=1$ and $\exists i \in P_1^j, S^i=1$, or  $x=0$ and $\exists i \in P_0^j, S^i=1$. That is to say,
% \bnm T^j  = (x\wedge\bigvee_{i\in P^j_1}S^i) \vee (\neg x\wedge\bigvee_{i\in P^j_0}S^i)  = (x\wedge\bigvee_{i\in P^j_1}S^i) \oplus (\neg x\wedge\bigvee_{i\in P^j_0}S^i)  \enm
% % The second equality follows from the identity that $(a\wedge b)\vee(\neg a \wedge c) = 
% % (a\wedge b)\oplus(\neg a \wedge c)$, for any bit variables $a, b, c$.  
% Because only one of the $S^i$ will be 1 at any time, therefore the inner OR gates can also be replaced with XOR:
% \bnm T^j  = (x\wedge\bigoplus_{i\in P^j_1}S^i) \oplus (\neg x\wedge\bigoplus_{i\in P^j_0}S^i), \; \text{ for } 1\le j\le q.\enm
% Therefore, each bit in $T$ requires at most $2$ AND gates to compute (assuming XOR gates can be computed without any garbling cost). To run $\dfa$ over a string of length $n$, we need to apply $\Trans$ $n$ times, and the resulting circuit contains no more than $2n\nstates$ AND gates.

% Finally, to check if the final state is accepted by $\dfa$, simply computing $\bigoplus\limits_{j\in\finalstates}S_n^j$ is sufficient.

%We omit the details of how to convert a regular expression into a DFA; the
%reader can refer to~\cite{chang1992regular} on how to so efficiently. 

% We currently support a subset of regular expressions. On restriction that we require is there should not be any overlapping matching substrings: once the DFA reaches an accepting state, no further matching should be possible. This can be achieved by having a 
% \todo{Or any manual modification we have done. This restriction is only applied to the second replacement protocol.}


% \paragraph{Representing $\trans$ as a Boolean circuit.}
% We represent each state as an one-hot encoding into a bit-vector of size
% $\nstates$, where $\state^j$ represents the $j$-the bit of the state $\state$.
% Without loss of generality, let assume $\state_0^j = 1$ for $j=1$, and
% $\state_0^j = 0$ for $1<j\le \nstates$. We note that exactly one location in the
% bit-vector is one for any state.  We also crate two sets for each state $j$, $P_0^j$ and $P_1^j$, where $P_b^j = \{i\suchthat\trans(i,b) = j\}$ for $b\in\zo$.


% We will now specify the transition function as a Boolean circuit. Let
% $t = \trans(s, x)$. we claim that $t^j=1$ if and only if either $x=1$ and $\exists i\in P_1^j, s^i=1$, or  $x=0$ and $\exists i\in P_0^j, s^i=1$. That is to say,
% \bnm t^j  = (x\wedge\bigvee_{i\in P^j_1}s^i) \vee (\neg x\wedge\bigvee_{i\in P^j_0}s^i)  = (x\wedge\bigvee_{i\in P^j_1}s^i) \oplus (\neg x\wedge\bigvee_{i\in P^j_0}s^i)  \enm
% The second equality follows from the identity that $(a\wedge b)\vee(\neg a \wedge c) = 
% (a\wedge b)\oplus(\neg a \wedge c)$, for all bit variables $a, b, c$.  Also, because only one of the $s^i$ will be 1 at any time, there fore the inner Or gates can be replaced with XOR.
% \bnm t^j  = (x\wedge\bigoplus_{i\in P^j_1}s^i) \oplus (\neg x\wedge\bigoplus_{i\in P^j_0}s^i), \; \text{ for } 1\le j\le n\enm

% We can apply the modified Boolean transition function $\trans$  to compute the final state $s_n = \transstring(\vecx)$, and to see if the final state is accepting or not we simply check if $\bigoplus\limits_{j\in\finalstates}s_n^j$ is 1 or not.
% This conversion ensures more number of XOR gates, which are more efficient to garble than AND gates.



% \paragraph{Garbled circuit size.} Each output bit of $\Trans$ requires at most $\nstates$ XOR gates and $2$ AND gates to compute. Therefore, each computation of $\Trans(\State, x)$ will take $\nstates^2$ XOR gates, and $2\nstates$ AND gates. Assuming the free XOR technique is applied, running DFA over a string of length $n$ will require the size of garbled circuit to be $\bigO(n\nstates)$.



% The message contains trigger data to describe the event. However, this doesn’t necessarily indicate the action will also be performed, since the user might add some additional checks on the trigger data. For example:

% \begin{itemize}
%     \item When the trigger is ``new SMS received", the rule might have some condition checks on the message text, such as whether it contains the word ``alert".
%     \item When the trigger is some time-sensitive condition such as ``the kid leave home", the rule might also add additional conditions such as ``which kid".
% \end{itemize}

% The execution diagram is shown in Fig \ref{exec_push} and the protocols for each party is described below:


% \paragraph{Trigger Service (\TS).} Once \TS has the trigger data $\dt$ and trigger payload $\payload$ ready, it selects a $j$ that has not been selected by previous executions and sets $(\ei_\dt, R, k) \gets e^{(j)}$. \TS executes the encoding protocol $$\LT \gets \En(\ei_\dt, \dt)$$ where $\LT$ is the labels of trigger data $\dt$ (similar to \TC's label generation procedure).

% Then, \TS records the current timestamp $t$ and computes $\Enc_k((j, t, \payload))$ using a symmetric-key encryption scheme. Finally, \TS sends $j$, $\LT$, and $\Enc_k((j, t, \payload))$ to \TAP. 


% \paragraph{Trigger-Action Platform (\TAP).} After receiving $j$, $\LT$, and $\Enc_k((j, t, \payload))$ from \TS, \TAP sets $(\Fone, \Ftwo) \gets F^{(j)}$ and $(C_1, C_2) \gets C^{(j)}$ and executes two evaluation protocols $$P \gets \Ev(\Fone, (\LT, C_1))$$ and $$Y \gets \Ev(\Ftwo, (\LT, C_2)),$$ where $P$ is the label of the predicate bit and $\LA$ is the labels of action data.

% Finally, \TAP passes $j, P, Y,$ and $\Enc_k((j, t, \payload))$ to \AS.

% \paragraph{Action Service (\AS).} After receiving $j$, $P$, $Y$, and $\Enc_k((j, t, \payload))$ from \TAP, \AS sets $(d_{f_1}, \Enc_{L_1^p}(d_{f_2}, k)) \gets d^{(j)}$. \AS first executes a decoding protocol
% $$ p \gets \De(d_{f_1}, P). $$

% If $p = 0$, \AS ignores the rest of the message and terminates the protocol. If $p = 1$, then $P = L_1^p$ and thus \AS can get $$(d_{f_2}, k) \gets \Dec_P(\Enc_{L_1^p}(d_{f_2}, k)).$$

% A second pair of decoding and decryption protocols is then executed to compute the action data $y$ and the payload $\payload$:
% $$ y \gets \De_H(d_{f_2}, Y) $$
% $$ (j', t', \payload) \gets \Dec_k(\Enc_k((j, t, \payload))) $$

% Finally, to ensure the integrity of the message, \AS needs to check if the following two conditions hold:
% \begin{itemize}
%     \item The unique identifier $j$ sent by \TAP equals to the unique identifier $j'$ selected by \TS,
%     \item $t - t' < \varepsilon$, where $t$ is the timestamp when the message is received by \AS and $\varepsilon$ is some predefined threshold.
% \end{itemize}

% \yc{Probably should use some algorithm boxes to represent the above protocols}








==> extra.tex <==
\begin{comment}
The main idea is that since, the view of the TS is computationally indistinguishable from the one generated by the simulator with no access to either the client inputs or the function outputs, no p.p.t adversary can violate the aforemnetioned privacy guarantee. 
 \begin{theorem} Let $View^{\Pi}_{TS}(f_1,f_2,x,\payload)$  and $Output_{TS}^{\Pi}(f_1,f_2,x)$ denote the view and output of the TS respectively. There exists a simulator $Sim_{TS}()$ such that \begin{gather}Sim_{TS}\equiv_c (View^{\Pi}_{TS}(f_1,f_2,x,\payload),Output_{TS}^{\Pi}(f_1,f_2,x))\end{gather} where $\equiv_c$ denotes computational indistinguishability. \end{theorem}
 \begin{proof}The view of the TS is given by \begin{gather} View^{\Pi}_{TS}(f_1,f_2,x,\payload) = \langle  e_x, R, k \rangle \\ Output^{\Pi}_{TS}(f_1,f_2,x,\payload) = \langle j, X, \Enc_k(j,t,\payload) \rangle \end{gather} 
 \end{proof}
 \end{comment}}
 
 
 
   \begin{comment}{
    \underline{$\privone$:}\\[2pt]
    \mytab $\left(f, (\dt^0, \const^0, \dtp^0), (\dt^1, \const^1, \dtp^1)\right)\getsr \adv $\\
    \mytab If $f(\dt^0, \const^0) \ne f(\dt^1, \const^1)$ then \ Return $\false$\\
    % \mytab $f\getsr \adv $\\
    % \mytab $M^0:=\{x^0,c^0,\payload^0\} \getsr \adv$\\
    % \mytab $M^1:=\{x^1,c^1,\payload^1\} \getsr \adv \mbox{ s.t }$\\
    % \mytab $\De'(d,\Ev(F,(X^0,C^0))) = \De'(d,\Ev(F,(X^1,C^1))) $\\
    \mytab $b\getsr\zo$\\
    \mytab $\mbox{ Pick } j$\\
    \mytab $\sects\getsr \{0,1\}^\kappa$\\
     \mytab $\secas\getsr \{0,1\}^\kappa$\\
    \mytab $(j,F,C,\encd) \getsr \textsf{CktGarbling}\left((f,c^b),(j,\sects,\secas)\right)$\\
    \mytab $(j, X, ct) \getsr \textsf{TriggerExec}((x^b,\payload^b), (\sects,j))$\\
    \mytab $(j,Y, ct,\encd) \gets \textsf{PlatformExec}\left((j,X, ct), (F, C,\encd)\right)$\\
    \mytab $b'\getsr \adv(j,\encd,Y,ct)$\\
    $\return b=b' $
  }\end{comment}

==> images/tap-image.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
  % uncomment if require: \path (0,350); %set diagram left start at 0, and has height of 350

  % Rounded Rect [id:dp1785865898985859]
  \draw   (220,38) .. controls (220,33.58) and (223.58,30) .. (228,30) -- (282,30) .. controls (286.42,30) and (290,33.58) .. (290,38) -- (290,62) .. controls (290,66.42) and (286.42,70) .. (282,70) -- (228,70) .. controls (223.58,70) and (220,66.42) .. (220,62) -- cycle ;
  % Rounded Rect [id:dp7261388468309096]
  \draw   (220,143) .. controls (220,138.58) and (223.58,135) .. (228,135) -- (282,135) .. controls (286.42,135) and (290,138.58) .. (290,143) -- (290,167) .. controls (290,171.42) and (286.42,175) .. (282,175) -- (228,175) .. controls (223.58,175) and (220,171.42) .. (220,167) -- cycle ;
  % Rounded Rect [id:dp4566547980113821]
  \draw   (50,144) .. controls (50,139.58) and (53.58,136) .. (58,136) -- (112,136) .. controls (116.42,136) and (120,139.58) .. (120,144) -- (120,168) .. controls (120,172.42) and (116.42,176) .. (112,176) -- (58,176) .. controls (53.58,176) and (50,172.42) .. (50,168) -- cycle ;
  % Rounded Rect [id:dp9714725640883546]
  \draw   (418,142) .. controls (418,137.58) and (421.58,134) .. (426,134) -- (480,134) .. controls (484.42,134) and (488,137.58) .. (488,142) -- (488,166) .. controls (488,170.42) and (484.42,174) .. (480,174) -- (426,174) .. controls (421.58,174) and (418,170.42) .. (418,166) -- cycle ;
  % Straight Lines [id:da5497844326272198]
  \draw    (215,68) -- (120.66,131.88) ;
  \draw [shift={(119,133)}, rotate = 325.9] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
  % Straight Lines [id:da3961070097617493]
  \draw    (251,75) -- (250.03,132) ;
  \draw [shift={(250,134)}, rotate = 270.97] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
  % Straight Lines [id:da004539666322914249]
  \draw    (296,68) -- (436.15,126.23) ;
  \draw [shift={(438,127)}, rotate = 202.56] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
  % Straight Lines [id:da6588770815496318]
  \draw    (127,154) -- (213,153.02) ;
  \draw [shift={(215,153)}, rotate = 539.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
  % Straight Lines [id:da08992770814603812]
  \draw    (296,154) -- (412,154) ;
  \draw [shift={(414,154)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

  % Text Node
  \draw (255,50) node   [align=left] {Mobile\\Client};
  % Text Node
  \draw (255,155) node   [align=left] {TAP};
  % Text Node
  \draw (85,156) node   [align=left] {Trigger\\Service};
  % Text Node
  \draw (453,154) node   [align=left] {Action\\Service};
  % Text Node
  \draw (126,84) node    {$j,e^{( j)} ,k_{j}$};
  % Text Node
  \draw (306,117) node    {$j,F^{( j)} ,A^{( j)}$};
  % Text Node
  \draw (401,71) node    {$j,\ E_{L^{o,( j)}_{1}}\left( d^{( j)}_{2} ,k_{j}\right)$};
  % Text Node
  \draw (95,209) node    {$ \begin{array}{l}
                              X\leftarrow \En\left( e^{( j)} ,x\right)\\
                              C\leftarrow E_{k_j}( x_{p})
                            \end{array}$};
                          % Text Node
                          \draw (271,216) node    {$ \begin{array}{l}
                                                       Y_{1}\leftarrow \mathsf{Ev}\left( F^{( j)}_{1} ,X\right)\\
                                                       Y_{2}\leftarrow \mathsf{Ev}\left( F^{( j)}_{2} ,X\right)
                                                     \end{array}$};
                                                   % Text Node
                                                   \draw (167,141) node    {$j,X,C$};
                                                   % Text Node
                                                   \draw (346,170) node    {$j,Y_{1} ,Y_{2} ,C$};
                                                   % Text Node
                                                   \draw (503,256) node    {$ \begin{array}{l}
                                                                                r\leftarrow D_{Y_1}\left( E_{L^{o,( j)}_{1}}\left( d^{( j)}_{2} ,k_{j}\right)\right)\\
                                                                                \mathrm{if} \ r\neq \bot \mathrm{then} \ \\
                                                                                \ \ \ \ \ \left( d^{( j)}_{2} ,\ k_{j}\right)\leftarrow r\\
\ \ \ \ \ y\leftarrow De\left( d^{( j)}_{2} ,Y_{2}\right)\\
\ \ \ \ \ x_{p}\leftarrow D_{k_j}( C) \ \\
\end{array}$};


\end{tikzpicture}


==> security2.tex <==
\section{Security Analysis of \stap}
\label{sec:sec_analysis}

\begin{figure*}[t]
  \tabfontsize\centering
%  \fpage{0.35}{
  \hfpagesss{0.315}{0.31}{0.31}{
    \underline{$\obliv$:}\\[2pt]
    $\left(f, (\dt^0, \const^0, \dtp^0), (\dt^1, \const^1, \dtp^1)\right)\getsr \adv $\\
    % $M^0:=\{x^0,c^0,\payload^0\} \getsr \adv$\\
    % $M^1:=\{x^1,c^1,\payload^1\} \getsr \adv$\\
    $\mbox{Pick } j$ ;\; $\sects\getsr \{0,1\}^\kappa$ ;\; $\secas\getsr \{0,1\}^\kappa$\\
    $b\getsr\{0,1\}$\\
    $j,F,C,\encd \getsr \cktgarbling\left((f,c^b), (\sects,\secas,j)\right)$\\
    $j,X,ct \getsr \tsexec\left((x^b,\payload^b),(\sects, j)
    \right)$\\
    $b'\getsr \adv(j,X,ct, F, C, \encd)$\\
    $\return b=b' $
   }{ %\\[2pt]
%  \fpage{0.35}{
    \underline{$\auth$:}\\[2pt]
    $\left(f, (\dt, \const, \dtp)\right)\getsr \adv $\\
    % $ M:=\{x,c,\payload\} \getsr \adv$\\
    $\mbox{Pick } j$ ;\; $\sects\getsr \{0,1\}^\kappa$ ;\; $\secas\getsr \{0,1\}^\kappa$\\
    $j,F,C,\encd \getsr \cktgarbling\left((f,c),(j,\sects,\secas)\right)$\\
    $j,X,ct \getsr \tsexec\left((x,\payload),(\sects,j) \right)$\\ 
    $j', \Ytilde, ct', \encd'\getsr  \adv(j,X,ct, F, C, \encd)$\\
    $y' \gets \asexec\left((j',\Ytilde,ct',\encd'),\secas\right)$\\
    $\return (j', \Ytilde, ct', \encd') \ne (j, F(X), ct, \encd)$\\
    $\mytab\mytab \wedge y'\ne \bot $
    % $\return (\Ytilde \ne F(X) \mbox{ or } ct'\ne ct) \mbox{ and } y' \ne \perp $
  }    {%\\[2pt]
%  \fpage{0.35}{
    \underline{$\privone$:}\\[2pt]
    $\left(f, (\dt^0, \const^0, \dtp^0), (\dt^1, \const^1, \dtp^1)\right)\getsr \adv $\\
    If $f(\dt^0, \const^0) \ne f(\dt^1, \const^1)$ then \ Return $\bot$\\
    $\mbox{Pick } j$ ;\; $\sects\getsr \{0,1\}^\kappa$ ;\;$\secas\getsr \{0,1\}^\kappa$\\
    % $f\getsr \adv $\\
    % $M^0:=\{x^0,c^0,\payload^0\} \getsr \adv$\\
    % $M^1:=\{x^1,c^1,\payload^1\} \getsr \adv \mbox{ s.t }$\\
    % $\De'(d,\Ev(F,(X^0,C^0))) = \De'(d,\Ev(F,(X^1,C^1))) $\\
    $b\getsr\zo$\\
    $j,F,C,\encd \getsr \cktgarbling\left((f,c^b), (\sects,\secas,j)\right)$\\
    $j, X, ct \getsr \tsexec\left((x^b,\payload^b), (\sects, j)\right)$\\
    $j, Y, ct, \encd \gets \tapexec\left((j, X, ct), (F, C, \encd)\right)$\\
    %If $\textsf{ActionExec}\left((j,\encd,Y,ct),j-1\right)=\bot$ then Return $\bot$\\
    $b'\getsr \adv(j,Y,ct,\encd)$\\
    $\return b=b' $
  }
  \caption{Security games for \name.}
  \label{fig:games}
\end{figure*}

%\ef{formally discuss the security definitions, and introduce proof results}
In this section, we show that \stap meets the security goals outlined
in~\secref{sec:threat} by providing concrete security definitions and proofs.
% We denote our protocol for \stap by $\proto$.
We assume the adversaries are probabilistic polynomial time (ppt) ---
they % $\advA$ (malicious) and $\advB$ (semi-honest)
run in time polynomial in security parameter $\keylen$. The garbled circuit protocol $\G$ used in \name provides \emph{output privacy}, \emph{message obliviousness}, and
\emph{execution authenticity}. The encryption scheme $\ske$ is
\textsf{IND-CCA} secure. We model the hash function $\H$ as a random
oracle~\cite{RO}. Let $\negl(\cdot)$ to be a negligible function. 

We prove the security of each component of \name, namely TAP, TS, and AS, separately. The
security games are defined in~\figref{fig:games}. We provide proof sketches in
this section and defer the complete proof to~\appref{app:security}.


% For the rest of the discussion, we denote the protocol executed by \name by $\Pi$. Additionally, we assume that $\adv$ represents a p.p.t adversary. 

% In this section, we provide the formal security analysis for the three entities of \name -- TS, TAP and AS.

%\subsection{Security definitions.}
\subsection{Security against malicious TAP}
Following our threat model we assume the TAP is compromised and
\emph{malicious}. % Recall that our threat model assumes a \emph{malicious}
% adversary model where adversary $\advA$ compromised \TAP.
The security definitions we expect from \stap is as follows.

\paragraph{Obliviousness.}
We define obliviousness property of $\stap$ by the security game $\obliv$ as
shown in~\figref{fig:games}.  Informally, $\advA$ despite arbitrarily deviating
from the protocol should not know anything about the user-provided constants
$\const$, the trigger data $\dt, \dtp$, and the output of the function
$y \gets f(x)$.
% \begin{enumerate}
%    \item the input of the client, namely $\{c_1,c_2\}$ \item the input of TS, namely $x$ and $\payload$ \item the function outputs $p=f_1(x,c_1)$ and $y=f_2(x_,c_2)$
% \end{enumerate}
%Let $\mathcal{A}$ denote a p.p.t adversary. 
%Formally %\vspace{2em}

\begin{theorem}[TAP Obliviousness]
  For any ppt adversary $\advA$, the probability that $\advA$ wins the $\obliv$
  game is negligible. \bnm \Prob{\obliv = 1}\leq 1/2+\negl(\keylen)\,,\enm
  % $\negl(\cdot)$ is a negligible function and $\keylen$ is the security
  % parameter.
  \label{thm:TAP1}
\end{theorem}\vspace{-0.1in}
\noindent\textbf{Proof sketch.} The proof of this theorem follows directly
from the \emph{message obliviousness} security guarantee of garbled circuits
$\G$~\cite{zahur2015two} and the semantic security of the encryption scheme
$\ske$. As such, the attacker learns nothing about $(\dt, \payload, c)$ from
$(X, C, ct)$.  The formal proof is presented in~\appref{app:security}.


We achieve security against a malicious \TAP even with a GC implementation
for the semi-honest model. Recall that the ``generators'' --- the trusted client
(TC) and the trigger service (TS) --- in \name are at least semi-honest.  Hence, 
a valid garbled circuit for the correct function $f$ is always generated (as
\TC is trusted), and all inputs are correctly encoded (since \TS is semi-honest
and the ``evaluators'' \TAP and \AS have no input).  Thus, the only way a
malicious \TAP can compromise the security of \name is by forging an inauthentic
output label or by replaying, delaying, or dropping a message.  We
discuss \name's resilience to such attacks next.

\paragraph{Authenticity.} The security guarantee \textit{authenticity} ensures
that no ppt adversary can create a garbled output $\Ytilde\ne Y$ such that \AS
acts on $\Ytilde$ (that is to say $\asexec$ outputs anything but $\bot$ or $\false$).  The formal definition is given by the security game $\auth$
as shown in~\figref{fig:games}.

\begin{theorem}[TAP authenticity]
  For any ppt adversary $\advA$, the probability that $\advA$ wins the 
  game $\auth$ is negligible, \bnm \Prob{\auth = 1}\leq \negl(\keylen)\,. \enm 
  \label{thm:TAP2}
\end{theorem}\vspace{-0.1in}
\noindent\textbf{Proof sketch.} The proof follows from the non-malleability 
guarantee (IND-CCA) of the encryption scheme $\ske$, execution authenticity of
$\G$~\cite{zahur2015two}, and the collision resistance of the hash function
$\H$. The full proof is presented in~\appref{app:security}.

\paragraph{Protection from altering the timing of rule execution.}  An adversary
cannot forge a message that the \AS will accept due to the strong authenticity
guarantee of \stap protocol. However, it can alter the execution time of a rule
by deliberately dropping, delaying, or replaying messages. \TAP can successfully drop a message without being detected by \AS. However, this would fall under the denial-of-service attack which is beyond \name's scope (\secref{sec:threat}). \name also protect against replayed or delayed messages. % In the following
% paragraphs, we discuss \name's course of action for the above mentioned
% attacks.% . We informally state guarantees that \name
% provide to defend against three types of attacks: delay in delivery, dropping a
% message and message replay.
% as shown by the following theorem.  \name defends against the following
% attacks from \TAP \begin{enumerate}\item delay a message \item replay a
%   message \item tamper a message \end{enumerate} \end{theorem}

% First, % $\stap$ protect against a delay in message delivery.
Every message from \TS is timestamped as they are sent which $\AS$ can check before performing any action. Therefore,
\AS will reject a message --- outputting $\bot$ ---  if the received message is delayed more than $\delay$ seconds (a parameter set by \AS) since
the time it was sent from \TS. (See the function \textsf{ASExec}
in~\figref{fig:algo}.) % Recall that, before acting upon any action message, the AS checks the freshness of the message, $t'-t\leq \delta$ (\textsf{ActionExec} in Figure ~\ref{fig:algo}).
% Therefore, $\adv$ cannot delay the message more than $\delay$ seconds (a
% parameter in the system set by \AS). This also prevents an adversary who
% compromised the TAP to replay a message older than $\delay$ seconds. 
We
acknowledge that the TAP can replay any message for which $\fone(x, c) = \false$
without getting detected by the AS.

\paragraph{Tampering with circuit id $j$.}
\change{The malicious TAP can modify the circuit id $j$ --- an unique identifier
  given to every instance of a garbled circuit for synchronization between TAP,
  TS, and AS --- in whatever way they want to. But \name ensures AS will always
  be able to detect any such modification and rejects the message from TAP (by
  outputting $\bot$).  This is done by having TS include the circuit id $j$ in
  the encrypted payload $ct$ --- that TAP cannot modify. AS, verifies that
  value against the circuit id forwarded by TAP, and any mismatch results in
  execution termination. 
% This ID specifies which circuit the \TAP should execute in response to a message from the \TS. All parties (\TS, \TAP, \AS) will learn about this index value and this can lead to metadata attacks on rules where encryption is not sufficient to protect the message contents (e.g., time-sensitive rules described in ~\secref{sec:supported-functions}). However, as specified in our threat model, these rules are only a small-fraction of the real-world rules that people actually use. Furthermore, because the \TAP is the party-in-the-middle for all rule executions, it can launch metadata attacks by simply observing message arrival patterns. Thus, knowledge of the circuit id \emph{does not grant the \TAP any additional power} in launching metadata attacks.}
%
% A malicious \TAP could tamper with the circuit id.
%   This can lead to two situations: (1) The \TAP tries to move the index backwards and use old circuits; however, circuit execution will fail because the \TS will transmit labels for the true circuit and not the old one, leading to a denial of service. (2) The \TAP tries to move the index forwards, thus exhausting circuits, leading again, to a denial of service. As specified in ~\secref{sec:threat}, denial of service is outside the scope of our work. 
% We note that this could allow \TAP to trick \TC to generate and send more circuit than required and propose a defense relying on synchronization with TS in ~\secref{sec:discussion}.
%
  Though TAP cannot tamper with $j$ without being detected, TAP could learn popularity of certain rules by observing circuit id values (which is passed to TAP in plaintext to help find corresponding garbled circuit $F$ to execute).  We acknowledge that metadata attacks are a limitation in \name and we discuss a cover traffic approach to address them (\secref{sec:discussion}).
  % This incurs a trade-off in network bandwidth consumption and processing on the \TAP.
}


%
% In case \TAP replays a previously generated message where the predicate function $\fone(X,C)=\true$, \AS can detect this from the time stamp in the message (in $ct$) and the current time stamp.
% However, \TAP can replay messages labels from previous runs where $\fone(X,C)=\false$. 
But this does not lead to any undesirable outcome in practice because in this case \AS performs no action. Note that the above attack (replay of $\false$ labels) could have been prevented by keeping track of the last seen circuit id of each rule at \AS. However, maintaining such state information would violate the RESTfulness of \AS and hence, we decide against it. 

%The circuit ids are monotonically increasing consecutive numbers. \AS keepstrack of the circuit id of the previous successful rule execution, $\jprev$. Itwill not accept a new message where the circuit id $j\le\jprev$. Thus theattacker cannot replay a previous message or drop a message without beingdetected by \AS.

% Protection from message replay is also straight forward, as AS deletes the key
% and decoding information for a circuit index $j$ after use. The one-time use
% guarantees that $\adv$ cannot replay a previous message. Also, the adversary
% cannot manipulate the circuit index $j$, as else \textsf{ActionExec} will use
% wrong key $\payloadk$ and the decoding information $\encd$, and the function will fail anyway.

% In the function \textsf{ActionExec}, \AS checks whether the received circuit id
% is one more than the last seen id. In case this check fails, \AS can detect that
% $\adv$ might have dropped a message.


% is from The client uses a different key every time. Thus, if a message is replayed then the decryption key used by the \AS is different from the one used in encrypting the message (an old key is used). So decryption will fail due to the \textsf{IND-CCA} guarantee of the encryption scheme.\\
% \textbf{Case 3. Tamper a message}\\
% Any tampering of the message is prevented by the \textit{authenticity} security
% guarantee (Theorem
% ~\ref{thm:TAP2}).% will be defended against by the \textsf{IND-CCA} guarantee of the encryption scheme.

\subsection{Security Analysis of TS and AS}\label{sec:sec-ts}
We assume \TS and \AS are honest, but curious. We define security as follows.

% \paragraph{Privacy from \TS.} % $\TS$ should not learn anything about the user constants
% beyond what is revealed through $\f$. 
% \begin{comment}\begin{theorem}[$\privts$] Let $\viewts(\f,\dt,\dtp)$ and
%   $\outputts(\f,\dt,\dtp)$ denote the view and output of the \TS,
%   respectively. There exists a simulator $\simulator_{\TS}(j)$ such that
%   \bnm\simulator_\TS(j)\equiv_c
% \left(\viewts(\f,\dt,\dtp),\outputts(\f,\dt,\dtp)\right)\,,\enm where $\equiv_c$
% denotes computational indistinguishability. \label{thm:TS} \end{theorem}
% \end{comment}
\begin{theorem}[$\privts$] \TS does not learn anything about the user constants $(\cone,\ctwo)$. \label{thm:TS} \end{theorem}
\noindent\textbf{Proof Sketch.}
\TS only receives from the client $\sects$ and $j$, which it uses to compute the
seed $\ei=(\eis,\eir)$. Thus, it can only learn the pairs of labels for all the
input wires (including the ones for user constants) to the garbled
circuit. \TS, \emph{by design}, does not have access to the client constants.\\[-5pt]


% that the TS should not learn anything about the input of the client, namely
% $c$. We define this more formally in the following theorem. The main idea is
% that since the view of the \TS is computationally indistinguishable from the one
% generated by the simulator with no access to the client inputs, no p.p.t
% adversary can violate the aforementioned privacy guarantee.

% \paragraph{Privacy from \AS.}
\AS should not learn about the user constants and the trigger data beyond what
is revealed from the output of the function~$f$.  Let $y_1=\fone(x,c)$ and
$y_2=\ftwo(x,c)$. We also need to ensure that when the output of the predicate
function $y_1=\false$, \AS does not learn the output of the
function $\ftwo$ and the payload $\dtp$.  We formally state these properties,
using the theorem below.
\begin{theorem}[$\privas^0$] If $y_1=\false$, then \AS learns nothing about $(x,c,\payload)$ other than what is revealed from $y_1=\false$. \label{thm:AS1} \end{theorem}
\noindent\textbf{Proof.}  To know the value of $y_2$, \AS needs access to the decoding table
 $d'$ (from the \textit{obliviousness} guarantee of garbled circuits
 in~\cite{zahur2015two}).  \AS will be able to do this only if it has access to $L_1^{w_0}$ (from the IND-CCA security of the encryption
 scheme). Note, $L_1^{w_0}$ is available to \TAP, and subsequently to \AS, only if
 $\fone(\dt)=\true$ \cite{zahur2015two}. In case \TAP returns some garbage value other than $L_1^{w_0}$, the decryption still fails. Additionally, $\payload$ is protected by the IND-CCA security of the encryption
 scheme. 
% Further, the pre-image resistance of the hash function $\H$ prevents the \AS
% from learning the value of the XOR-offset $\eir$. Thus, the \AS has no way of
% figuring out $L_1^{w_0}$ and hence, the value of $y$ remains private from the
% \AS. 

\begin{comment}
  \begin{theorem}[$\privas$] Let $\viewas(\fone,\ftwo)$ and $\outputas(\fone,\ftwo)$ denote the view and the output of \AS respectively
  in protocol $\Pi$. For any $\dt, \dtp$, there exists
  a simulator $\simaszero(\fone, \ftwo, j, \fonev\cdot\ftwov, \fonev\cdot\dtp)$ such that \begin{gather*}
  \hspace{-3cm}\simaszero(\fone, \ftwo, j, \fonev\cdot\ftwov, \fonev\cdot\dtp) \\\hspace{2cm}\equiv_c\viewas(\fone,\ftwo), \outputas(\fone,\ftwo)
  \end{gather*}
  where $\equiv_c$ denotes computational
  indistinguishability, and $a\cdot b$ denotes $b$ if $a=\true$ and $\bot$ otherwise.\label{thm:AS} \end{theorem}
\noindent\textbf{Proof sketch.} The main idea of the proof is that the view of \AS is computationally indistinguishable from a tuple of ``random''  numbers, because of the  \textit{message obliviousness} guarantee of garbling scheme $\G$,
% in~\cite{bellare2012foundations},
the semantic security of the encryption scheme $\ske$, and the pre-image resistance of the hash function $\H$. Hence, $\simaszero(\fone, \ftwo, j,\fonev, \fonev\cdot\ftwov, \fonev\cdot\dtp)$  (which clearly has access to $\ftwov$ and $\dtp$ only when $y_1=1$) is able to ``simulate'' the view of \AS  without having access to the user constants and trigger data. The full proof is presented in the Appendix~\ref{app:security}. 
\end{comment}
% \rcnote{Talk about what is the simulator is doing here, and how that is giving us the coveted security.}

% \begin{comment}
% In order to know the value of $y$, the \AS needs to access the decoding table
% $d$ (from the \textit{obliviousnes} guarantee of garbled circuits
% in~\cite{bellare2012foundations}).  The \AS will be able to do this only if it
% has access to $L_1^{w_0}$ (from the IND-CCA security of the encryption
% scheme). Note, the value of the label is only available to \TAP when
% $\fone(\dt)=\true$, following the obliviousness property of the garbled circuit.
% Further, the pre-image resistance of the hash function $\H$ prevents the \AS
% from learning the value of the XOR-offset $\eir$. Thus, the \AS has no way of
% figuring out $L_1^{w_0}$ and hence, the value of $y$ remains private from the
% \AS. 
% \end{comment}


% \paragraph{$\text{Privacy}^1_{AS}$.} Informally, the $Privacy^1_{AS}$ guarantee states that if $p=1$, the \AS should not learn anything about
% \begin{enumerate}\item the input of the client, namely $(c_1,c_2)$ \item the input of \TS, namely $(x,\payload)$ \end{enumerate}
% except from what can be learned from the outputs $p=1$ and $y=f_2(x,c_2)$.
% We define this more formally via  the security game $\textsf{Priv}
% ^1_{\mathcal{A},\Pi}$ as shown in Figure~\ref{fig:games}.


\begin{theorem}[$\privas^1$] If $y_1=\true$, then for any ppt adversary $\advB$, the probability that
  $\advB$ wins the game $\privone$ is negligibly more than random guessing. That is,
  \bnm \Prob{\privone = 1}\le 1/2 + \negl(\keylen)\,.\enm \label{thm:AS2}
\end{theorem}\vspace{-0.1in}
\noindent\textbf{Proof sketch.}  The proof of the above theorem follows directly from the
\textit{input privacy} guarantee provided by garbled
circuits~\cite{zahur2015two} and the semantic security of the
encryption scheme. The full proof is presented in Appendix \ref{app:security}.


 %\begin{theorem}A p.p.t adversary $\adv$ satisfies the $\textit{Privacy}_{TS}$ guarantee in \name. \end{theorem}

 












% \begin{comment}
% \begin{figure}
% \begin{center}
% \fbox{
% \pseudocode{%
% \textbf{ Challenger} \< \< \hspace{-1.5cm}\textbf{ Adversary}  \\[0.1\baselineskip][\hline]
%  \<\< \\[-0.5\baselineskip]
% \<\<  f \\
% \<\< \hspace{-1cm}M^0=\{x^0,c^0,\payload^0\} \\
% \<\< \hspace{-1cm}M^1=\{x^1,c^1,\payload^1\} \\
%  \< \hspace{-1cm}\sendmessageleft*{f,M^0,M^1} \< \\
% b \getsr\{0,1\} \< \< \\
% k\getsr \skegen(1^\kappa) \< \< \\  e \getsr \{0,1\}^{2\cdot\kappa}\< \< \\ (F,d) \leftarrow \Gb'(f,e)\< \< \\ j, t \< \< \\ C^b\leftarrow \En(e,c^b)\< \< \\ X^b \leftarrow 
%  \En(e,x^b) \< \< \\ ct^b \getsr \skeenc(k, (t, \payload^b))\< \<\\
%  \< \hspace{-1cm} \sendmessageright*{j,F,X^b,C^b,ct^b} \< \\
%  \<\< \hspace{-0cm}b' \in \{0,1\} \\
%  \< \hspace{-1cm}\sendmessageleft*{b'} \< \\
% \< \textsf{Obliv}_{\mathcal{A},\Pi} = 1 \mbox{ if } b'= b \< }
% }\vspace{0.5cm}
% \end{center}

% \end{figure}
% \end{comment}



% \begin{enumerate}\item Adversary $\mathcal{A}$ outputs functions $f_1$ and $f_2$, and a pair of message tuples  $M^0=\{x^0,c^0_1,c^0_2,\payload^0\}$ and $M^1=\{x^1,c^1_1,c^1_2,\payload^1\}$.
% \item $\Pi$ generates key $k\getsr \skegen(1^\kappa)$, $e:=\langle e_s,e_r \rangle \getsr \{0,1\}^{2\cdot\kappa}$ and  $(F_1,F_2,d_{f_1},d_{f_2}) \leftarrow \Gb'(f_1,f_2,e)$. 
%  Next, $\Pi$ picks a uniform bit $b$, selects values $j$ and $t$, and computes $C^b_1\leftarrow \En(e,c^b_1), C^b_2\leftarrow \En(e,c^b_2), X^b \leftarrow 
%  \En(e,x^b)$. Finally, it sends $(j,F_1,F_2,X^b,C^b_1,C^b_2,\skeenc(k,(j,t,\payload^b)))$  to $\mathcal{A}$. \item  $\mathcal{A}$ outputs a bit $b'$.
%  \item The output of the game is defined to be $1$ if $b' = b$,
% and $0$ otherwise. We write $\textsf{Obliv}
% _{\mathcal{A},\Pi} = 1$ if the output of the 
% game is $1$ and in this case we say that $\mathcal{A}$ succeeds. 
% \end{enumerate}
% \end{comment}


% \begin{comment}
% \begin{figure}
% \begin{center}
% \fbox{
% \pseudocode{%
% \textbf{ Challenger} \< \< \hspace{-1.5cm}\textbf{ Adversary}  \\[0.1\baselineskip][\hline]
%  \<\< \\[-0.5\baselineskip]
% \<\< \hspace{-0cm} f \\
% \<\< \hspace{-1cm}M=\{x,c,\payload\} \\
%  \< \hspace{-0.5cm}\sendmessageleft*{f,M} \< \\
% k\getsr \skegen(1^\kappa) \< \< \\  e \getsr \{0,1\}^{2\cdot\kappa}\< \< \\ (F,d) \leftarrow \Gb'(f,e)\< \< \\ j, t \< \< \\ C\leftarrow \En(e,c)\< \< \\ X \leftarrow 
%  \En(e,x) \< \< \\ ct \getsr \skeenc(k, (t, \payload))\< \<\\
%  \encd \getsr \skeenc(L^{w_0}_1, (d, k))\< \<\\
%  \< \hspace{-0.5cm} \sendmessageright*{j,F,X,C,ct} \< \\
%  \< \hspace{-0.5cm}\sendmessageleft*{Y'} \< \\
% \<\hspace{-1cm}  \textsf{Auth}_{\mathcal{A},\Pi} = 1 \mbox{ if } \textsf{ActionExec}((Y',ct),(\encd))\neq \perp \< }
% }
% \end{center}
% \caption{$\textsf{Auth}_{\mathcal{A},\Pi}$ security game}\label{fig:auth}
% \end{figure}

% \end{comment}



% \begin{comment}
% \begin{enumerate}\item Adversary $\mathcal{A}$ outputs functions $f_1$ and $f_2$ and a message tuple $\{x,c_1,c_2,\payload\}$. \item $\Pi$ generates a key $k\getsr \skegen(\kappa)$,  $e:=(e_s,e_r)\getsr \zo^{2\kappa}$ and $(F_1,F_2,d_{f_1},d_{f_2}) \leftarrow \Gb'(f_1,f_2,e)$.  Next, it selects values $j$ and $t$, and computes $C_1\leftarrow \En(e,c_1), C_2\leftarrow \En(e,c_2), X\leftarrow \En(e,x)$ and sends $(j,F_1,F_2,X,C_1,C_2,\skeenc(k,(j,t,\payload))$ to $\mathcal{A}$. \item $\mathcal{A}$ outputs $\{P',Y', E'\}$
% \item $\mathcal{A}$ succeeds if and only if (1) $P'\neq \Ev(F_1,(X,C_1)) \wedge Y'\neq \Ev(F_2,(X,C_2))$ and (2) $\De'(d_
% {f_1},P')\neq\perp \wedge \De'(d_
% {f_2},Y') \neq\perp $ OR (1) $\skedec(k,E')=(j,t,\payload')$ and (2)$\payload'\neq \payload$. In this case the output of the game is defined to be 1.\end{enumerate}
% \end{comment}

% \subsection{Security Analysis for Action Service}
% %\arc{Still Working on it}
% We analyze the security against a compromised \AS in two phases. First when the
% output of $\fone(\dt, \const)$ is true, $\AS$ should not learn anything beyond
% $\f(\dt)$ and $\dtp$. When the output of $\fone(\dt, \const)$ is $\false$, \AS
% should not learn anything beyond that $\fone(\dt, \const)$ is false. 

% \paragraph{$\privzero$.} The first security requirement for the \AS states that, if $p=0$, then the \AS should learn nothing about \begin{enumerate}\item the input of the client, namely $(c_1,c_2)$ \item the input of \TS, namely $(x,\payload)$ \item the function output  $y=f_2(x,c_2)$ \end{enumerate}  except from what is revealed by the fact that $p=0$. This is proved by the following theorem. The main idea of the proof is that the \textit{view} of the \AS can be simulated by a simulator which has no access to  the inputs $(x,\payload,c_1,c_2)$ and $y$.


% \begin{theorem}The adversary $\mathcal{A}$ wins the $\textsf{Priv}^1_{\mathcal{A},\Pi}$ game with probability \begin{gather}\mbox{Pr}[\textsf{Priv}^1_{\mathcal{A},\Pi} = 1] \leq \frac{1}{2} + \textsf{negl}(\kappa)\end{gather} where $\textsf{negl}()$ is a negligible function and $\kappa$ is the security parameter. \end{theorem} 
% \paragraph{Proof Sketch.} The proof of the above theorem follows from the \textit{privacy} guarantee of garbled circuits~\cite{bellare2012foundations} and the semantic security of the encryption scheme. The full proof is presented in Appendix \ref{app:security}.




% \\\arc{Simpler version}
% \begin{theorem}If $p=0$, then the \AS has  no knowledge of $y=f_2(x,c_2)$. \end{theorem}









% \begin{comment}
% \begin{figure}
% \begin{center}
% \fbox{
% \pseudocode{%
% \textbf{ Challenger} \< \< \hspace{-1.5cm}\textbf{ Adversary}  \\[0.1\baselineskip][\hline]
%  \<\< \\[-0.5\baselineskip]
% \<\<  f \\
% \<\< \hspace{-1cm}M^0=\{x^0,c^0,\payload^0\} \\
% \<\< \hspace{-1cm}M^1=\{x^1,c^1,\payload^1\} \\
% \<\< \hspace{0cm}\mbox{ s. t.}  \\ \<\< \hspace{-2.5cm}\De'(d,\Ev(F,(X^0,C^0))) \\ \<\< \hspace{-2cm} = \De'(d,\Ev(F,(X^1,C^1)))
%  \< \<\\\<\hspace{-1cm}\sendmessageleft*{f,M^0,M^1} \< \\
% b \getsr\{0,1\} \< \< \\
% k\getsr \skegen(1^\kappa) \< \< \\  e \getsr \{0,1\}^{2\cdot\kappa}\< \< \\ (F,d) \leftarrow \Gb'(f,e)\< \< \\ j, t \< \< \\ C^b\leftarrow \En(e,c^b)\< \< \\ X^b \leftarrow 
%  \En(e,x^b) \< \< \\ ct^b \getsr \skeenc(k, (t, \payload^b))\< \<\\
%  Y^b=\Ev(F,(X^b,C^b))\<\<\\
%  \< \hspace{-1cm} \sendmessageright*{j,\encd,Y^b,ct^b} \< \\
%  \<\< \hspace{-0cm}b' \in \{0,1\} \\
%  \< \hspace{-1cm}\sendmessageleft*{b'} \< \\
% \< \textsf{Priv}^1_{\mathcal{A},\Pi} = 1 \mbox{ if } b'= b \< }
% }\vspace{0.5cm}
% \end{center}
% \caption{$\textsf{Priv}^1_{\mathcal{A},\Pi}$ security game}\label{fig:priv}
% \end{figure}

% \end{comment}






% \begin{comment}
%  \begin{enumerate}\item Adversary $\mathcal{A}$ outputs functions $f_1$ and $f_2$, and a pair of message tuples  $X^0=\{x^0,c^0_1,c^0_2,\payload^0\}$ and $X^1=\{x^1,c^1_1,c^1_2,\payload^1\}$ such that \scalebox{1}
%  {$\De'(d_{f_1},\Ev(F_1,(X^0,C^0_1))) = \De'(d_{f_1},\Ev(F_1,(X^1,C^1_1)))
%   \wedge$}  \scalebox{0.9}
%   {$ \De'(d_{f_2},\Ev(F_2,(X^0,C^0_2))) $}
%   \scalebox{0.9}{$ = \De'(d_{f_2},\Ev(F_2,(X^0,C^0_2)))$
%   }
% \item $\Pi$ generates a key $k\getsr \skegen(1^\kappa)$,  $e:=(e_s,e_r)\getsr \zo^{2\kappa}$ and $(F_1,F_2,d_{f_1},d_{f_2}) \leftarrow \Gb'(f_1,f_2,e)$. 
%  Next, $\Pi$ picks a uniform bit $b$, selects $j$ and $t$ and computes $C^b_1\leftarrow \En(e,c^b_1), C^b_2\leftarrow \En(e,c^b_2), X^b \leftarrow 
%  \En(e,x^b), P^b\gets\Ev(F_1,X^b,C^b_1), Y^b\gets\Ev(F_2,X^b,C^b_2)$ and $\tilde{d}:=(d_{f_1},\skeenc(L_1^p,(d_{f_2},k)))$. Finally, it sends $(F_1,F_2,j,\tilde{d},P^b,Y^b,\skeenc(k,(j,t,\payload^b)))$  to $\mathcal{A}$. \item  $\mathcal{A}$ outputs a bit $b'$.
%  \item The output of the game is defined to be $1$ if $b' = b$,
% and $0$ otherwise. We write $\textsf{Priv}_{\mathcal{A},\Pi} = 1$ if the output of the 
% game is $1$ and in this case we say that $\mathcal{A}$  succeeds.
% \end{enumerate}
% \end{comment}




% \begin{comment}

% \begin{proof}The indistinguishability of $\skeenc(k,(j,t,\payload^b))$ follows from the semantic security of the encryption scheme. The rest of the proof follows from proof for the corresponding game ($priv.ind$ with $\phi(f)=f$) in~\cite{bellare2012foundations}. In fact in our setting, the view of the $\adv$ is a strict subset of that of the adversary presented in ~\cite{bellare2012foundations}. Specifically, our advserary $\adv$ does not have access to the garbled inputs $X^b,C^b_1$ and $C^b_2$.   \end{proof}

% \end{comment} 

% The knowledge that trigger is fired already leak information about the
% sensitive data. For example, a smart door can send triggers ``on door open'', or
% ``on heater on''.
% However, as both string and arithmetic operations are represented as boolean
% circuit, combining them would not be



% Let the number of gates in the circuit be $r$, then $w_1,\ldots, w_m$ represents the
% input wires, and $w_{r-n+1},\ldots,w_{r}$ represents the output wires.  
% to

% \begin{itemize}
% \item \emph{The garbled circuit generation function ($\Gb$)} converts an
%   arbitrary function $f\Colon\zo^n\mapsto\zo^m$ (that can be expressed as a
%   Boolean circuit) into a garbled circuits $F$, an encoding information $e$, and
%   a decoding information $d$.  Therefore, $(F, e, d) \getsr \Gb(1^\keylen,
%   f)$. This function is performed by the trusted client during the rule setup
%   phase.
% \item \emph{The encoding function ($\En$)} takes as input the encoding
%   information $e$ and a bitstring $x\in\zo^n$ and returns a set of input labels
%   $X$. This function is deterministic and is performed by the trigger service.
% \item \emph{The garbled evaluation function ($\Ev$)} takes the garbled circuit $F$
%   and a set of input label $X$ as input and returns a set of output labels
%   $Y$. This function is deterministic and is performed by the TAP.
% \item \emph{The decoding function ($\De$)} takes in the decoding information $d$
%   and output labels $Y$ and returns the output bits $y$. This function is
%   deterministic and is performed by the action service.
% \end{itemize}

% The correctness guarantees of garbled circuit guarantees that\bnm \De( \Ev(F,
% \En(x, e)) , d) = f(x) \enm.%  , during the rule execution, the garbled operations
% % we perform on the trigger data are equivalent to the original function $f$:


% By applying the garbled circuit protocol, each bit in the trigger data becomes
% a random label, which is usually presented as a 128-bit string. However, by
% utilizing the point-and-permute optimization \cite{b12}, we can reduce the
% size of the output (action) label to 1 bit.




==> security_appen2.tex <==
\subsection{Security Analysis Contd.}\label{app:security}
%\arc{Some notational mismastch left, will fix}


\begin{customthm}{VI.1}[TAP Obliviousness]
  For any ppt adversary $\advA$, the probability that $\advA$ wins the $\obliv$
  game is negligible. \bnm \Prob{\obliv = 1}\leq 1/2+\negl(\keylen)\,,\enm
  \end{customthm}
\begin{proof} First, note that the game $\obliv$ is equivalent to the game $obv.sim_{\mathcal{S}}$ \cite{bellare2012foundations} in \cite{zahur2015two}. Now, consider the simulator $\mathcal{S}$ as presented in Fig. 3 in \cite{zahur2015two}. In our setting, $\mathcal{S}$  is used by \TC and \TS to generate $(\hat{F},\hat{X},\hat{C})$ which is then used for the rest of the computation. Hence the obliviousness of ($x,c$) follows directly from the corresponding proof (game $obv.sim_{\mathcal{S}}$) presented in \cite{zahur2015two} assuming the random oracle model for $\H$ \cite{RO}.  The indistinguishability of $ct^b$ follows trivially from the semantic security guarantee of the encryption scheme, thereby concluding our proof. \end{proof}


\begin{customthm}{VI.2}[TAP authenticity]
  For any ppt adversary $\advA$, the probability that $\advA$ wins the security
  game $\auth$ is negligible, \bnm \Prob{\auth = 1}\leq \negl(\keylen)\,. \enm 
 \end{customthm}
\begin{proof} The authenticity of $ct$ follows from the \textsf{IND-CCA} guarantee of the encryption scheme. 
For the rest of the proof, consider the simulator $\mathcal{S}$ in \cite{zahur2015two} which additionally returns $h=\H(\wlabel^{w_1}_0 \concat \ldots \concat \wlabel^{w_m}_0), e_r$ and $\wlabel^{w_0}_0$. \TC uses this additional information to generate the decoding blob $\encd$. Similarly, function in $\De$ \cite{zahur2015two} is changed to that of \textsf{ASExec}.

\noindent\emph{Case I: Authenticity of $y_1=\fone(x,c)$.}\\
Note that $\encs$ is encrypted under a key derived from $\secas$ and $\wlabel^{w_0}_0$. Hence, from the semantic security of the encryption scheme, \TAP does not have access to $e_r$ since it does not know $\secas$ by design. Thus, 
in case $y_1=\false$, \TAP has access only to the $\false$ label $\wlabel^{w_0}_0$ and thereby cannot cheat \AS. On the other hand, if $y_1=\true$, \TAP can return some garbage value $L'$ such that $\skedec(L'\xor\secas,\encd)=\bot$. However, \AS can detect this with the help of the $\textsf{HMAC}$. Moreover, %the use of $j$ in computing $\ench$ prevents \TAP from replaying any previously seen \textsf{HMAC}. Additionally, 
\TAP cannot send any of the hitherto unseen \textsf{HMAC}s  because it cannot obtain the output labels without access to  the corresponding $X$  (\TS's trigger data). \\

%The rest of the proof follows trivially from the corresponding proof (game $aut$)  in \cite{bellare2012foundations}. Note that, our garbled scheme compared functions slightly differently than the one presented in ~\cite{bellare2012foundations} (Scheme Garbled2) -- decoding table in our case is the hash digest of the output labels (Section~\ref{sec:arch}). However, due to the collision resistance of the hash function $\H$, the proof in \cite{bellare2012foundations} remains unaffected (specifically the check $\De'(d,L^{w_1},\cdots,L^{w_m})\neq \perp)$ 

\textit{Case II - Authenticity of $y_2=\ftwo(x,c)$. } \\  
From the collision resistance of $\H$, the only way \TAP can cheat is by generating a label $\wlabel^{w_i}_{1-y_2[i-1]}$ for some wire $i \in [1,m]$ where $y_2[i]$ denotes the $i$-th bit of $y_2$. However,  as discussed above, \TAP cannot compute any other label other than the one obtained from $\Ev(F,X,C)$.

The rest of the proof follows an identical sequence of hybrids as the proof of Theorem 1 in \cite{zahur2015two} assuming the random oracle model for $\H$. \end{proof}


 
\begin{customthm}{VI.5}[$\privas^1$] If $y_1=\true$, then for any p.p.t adversary $\advB$, the probability that
  $\advB$ wins the $\privone$ is negligibly more than random guessing. That is,
  \bnm \Prob{\privone = 1}\le 1/2 + \negl(\keylen)\,.\enm 
\end{customthm}
\noindent\textbf{Proof.} The indistinguishability of $ct^b$ follows from the semantic security of the encryption scheme.  Now note that $\privone$ is equivalent to $prv.sim_\mathcal{S})$ \cite{bellare2012foundations} in  \cite{zahur2015two}. The rest of the proof is based on the proof for the corresponding game ($prv.sim_\mathcal{S})$ in \cite{zahur2015two}). In fact in our setting, the view of the $\adv$ is a strict subset of that of the adversary presented in ~\cite{zahur2015two}. Specifically, our adversary $\adv$ does not have access to the garbled inputs $X^b,C^b$ and the garbled circuit $F$.  
Note that in the above game, a malicious \TAP instead of outputing $(Y, ct) \gets \textsf{TAPExec}\left((X, ct), (F, C)\right)$, could generate some arbitrary message. However, from the obliviousness property of garbled circuits (Thm. \ref{thm:TAP1}, we know that this message has to be  completely oblivious of $(F,X,c)$ and hence the privacy guarantee is upheld trivially. 




% \begin{comment}
%   \begin{customthm}{6.4} [$\privas$] Let $\viewas(\fone,\ftwo)$ and $\outputas(\fone,\ftwo)$ denote the view and the output of \AS 
%   in protocol $\Pi$ respectively. For any $\dt, \dtp$, there exists
%   a simulator $ \simulator_{\AS}( \fone, \ftwo, j, y_1, y_1\cdot y_2, y_1 \cdot \payload)$ such that \begin{gather*}
%   \hspace{-3cm}\simaszero(\fone, \ftwo, j, \fonev, \fonev\cdot\ftwov, \fonev\cdot\dtp) \\\hspace{2cm}\equiv_c\viewas(\fone,\ftwo), \outputas(\fone,\ftwo)
%   \end{gather*}
%   where $\equiv_c$ denotes computational
%   indistinguishability.\end{customthm}
% \begin{proof} For the following proof, we consider the random oracle model for $\H$ \cite{RO}. Let us first consider the case when $y_1 = 0 (\false)$. Let $Y=\langle Y_1,Y_2\rangle$ such that $Y_1=L^{w_0}$ and $Y_2=(L^{w_1},\cdots,L^{w_m})$. The view and the output of the \AS are given by
% \begin{gather}\viewas(f_1,f_2) = \langle j,  \tilde{d}, Y, ct, \secas \rangle  \\\outputas(f_1,f_2)=\perp\end{gather}  Here, the simulator $\simulator_{\AS}(f_1,f_2, j, 0,0,0)$, does not know the values of $\ftwov$ and $\payload$ (since $\fonev=0$) and performs the following operations \begin{enumerate}%\item selects $\sects'\getsr \{0,1\}^\kappa$ \item computes $e_s' \gets \H(\sects' \concat j\concat 0), e_r' \gets \H(\sects'\concat j\concat 1) \vee 0^{m-1}1$
% \item selects $Y_1'\getsr \{0,1\}^\kappa$ and $Y_2'\getsr \{0,1\}^{m\cdot \kappa}$ 
% \item selects $\secas'\getsr \{0,1\}^\kappa$
% \item selects $E_1' \getsr \{0,1\}^{3\kappa+|j|+|d|}$ such that $\textsf{D}\left((Y_1'\bigoplus \secas'), E_1'\right) = \perp$ (this can be ensured by making the authentication check fail)
% \item selects  $E_2' \getsr \{0,1\}^{|t|+|v|}$
% \end{enumerate}
% From the semantic security of the encryption scheme, we have  $Y'=\langle Y_1', Y_2' \rangle \equiv_c \langle Y_1,Y_2 \rangle= Y$,  $ E'_1 \equiv_c \skeenc(L_1^{w_0}\bigoplus \secas,(j,k,e_r,d,h)) =\tilde{d}$ and $E'_2 \equiv_c ct $.
% Hence, the tuple $\langle j, E_1',Y',E_2', \secas'\rangle $ is computationally indistinguishable from $\langle j, \encd, Y, ct, \secas \rangle$. 
% \\
% Now, let us consider the case when $y_1=1 (True)$.  The view and the output of the \AS are given by
% \begin{gather}\viewas(f_1,f_2) = \langle j,  \tilde{d}, Y, ct, \secas \rangle  \\\outputas(f_1,f_2)=\langle y_2, \dtp \rangle \end{gather}  Here, the simulator  $\simaszero(\fone, \ftwo, j, 1, y_2, \payload)$ knows the values $y_1$ and $\dtp$ performs the following steps, 
% \begin{enumerate}
% \item selects $\secas' \getsr \{0,1\}^\kappa$
% \item selects $\sects' \getsr \{0,1\}^\kappa$
% \item computes $e_r'\gets \H(\sects'\concat j\concat 1) \vee 0^{m-1}1$
% \item computes $k' \gets \H(\sects'\concat j\concat 2)$
% \item selects $ \forall i \in [0,m], {L_0^{w_i}}' \getsr \{0,1\}^\kappa$
% \item computes $\forall i \in [1,m], {L_1^{w_i}}' := {L_0^{w_i}}'\bigoplus e_r $
% \item computes $Y' = \{ {L_1^{w_0}}', {L_{y_2[1]}^{w_1}}' \concat \cdots \concat {L_{y_2[m]}^{w_m}}' \}$ where $y_2[i], i \in [1,m]$ represents the $i$-th bit of $y_2$
% \item computes $h'=  \H({L_0^{w_1}}'\concat\cdots\concat {L_0^{w_m}}')$
% \item computes the appropriate decoding table $d'$ using $\langle {L_0^{w_i}}', {L_1^{w_i}}' \rangle$ as the labels for the output values $0$ and $1$ respectively for the $i$-th wire \item compute $E_1'= \skeenc(
% {L_1^{w_0}}' \bigoplus \secas, (j, k', e_r', d', h'))$ 
% \item compute $t_c\gets \textsf{CurrentTime}(), E_2' = \skeenc (k', (t',v))$ s.t. $  t_c-T\leq t' \leq t_c$  \end{enumerate}

% Note that clearly, $(j,k',e_r',d',h')= \skedec( {L_1^{w_0}}'\oplus \secas', E_1')$ and $y_2 = \De\left(d',Y'\right)$. Moreover, $(t',v) = \skedec(k',E_2')$. These two results in addition to the semantic security of the encryption scheme guarantees that $Y' \equiv_c  Y$, $E_1' \equiv_c \encd$ and $E_2' \equiv_c ct$.   Hence, the tuple $\langle j, E_1',Y',E_2', \secas'\rangle $ is computationally indistinguishable from $\langle j, \encd, Y, ct, \secas \rangle$. The output tuple $\langle y_2, \dtp \rangle$ can be clearly computed from the view thereby concluding our proof. 
% \end{proof}
% \end{comment}

% \begin{comment}\begin{customthm}{6.5}[$\privas^1$] For any ppt adversary $\advA$, the probability that
%   $\advA$ wins the $\privone$ is negligibly more than random guessing. That is,
%   \bnm \Prob{\privone = 1}\le 1/2 + \negl(\keylen)\,.\enm \end{customthm}
 
% \begin{proof}The indistinguishability of $ct^b$ follows from the semantic security of the encryption scheme.  The rest of the proof is based on the proof for the corresponding game ($priv.ind$ with $\phi(f)=f$) in~\cite{bellare2012foundations}. In fact in our setting, the view of the $\adv$ is a strict subset of that of the adversary presented in ~\cite{bellare2012foundations}. Specifically, our adversary $\adv$ does not have access to the garbled inputs $X^b,C^b$ and the garbled circuit $F$.   \end{proof}

%  %\begin{customthm}{6.3} [$\privts$] Let $\viewts(\f,\dt,\dtp)$ and$\outputts(\f,\dt,\dtp)$ denote the view and output of the \TS,
%   respectively. There exists a simulator $\simulator_{\TS}(j)$ such that
%   \bnm\simulator_\TS(j)\equiv_c
% \left(\viewts(\f,\dt,\dtp),\outputts(\f,\dt,\dtp)\right)\enm where $\equiv_c$
% denotes computational indistinguishability. \end{customthm}
% \begin{proof}The view of the \TS is given by \begin{gather} \viewts(f_1,f_2,x,\payload) = \langle  j, \sects\rangle \\ \outputts(f_1,f_2,x,\payload) = \langle e_s,e_r, \payloadk, X, ct \rangle 
%  \end{gather} 
%  %The output of the \TS can be generated from the view.
%  The simulator $\textsf{Sim}_{\TS}(j)$ samples $\sects'\getsr \{0,1\}^{\kappa}$. Seeds $e_s', e_r'$ and key $\payloadk'$ can be computed from $\sects'\concat j$ using the hash function $\H$. Next, use $e_s', e_r'$  to compute $X'\gets \En(e_s',e_r',x)$. Let $t\gets \textsf{CurrentTime()}$. Thus, the tuples $(\langle j,\sects'\rangle,\langle e_s', e_r', \payloadk', X',\E(\payloadk',(t,\dtp))\rangle)$ and $(\langle  j, \sects\rangle, \langle e_s, e_r, \payloadk ,  X, ct \rangle)$ are computationally indistinguishable from each other.\end{proof}
%  \end{comment}
% \end{comment}
